Subexponential Parameterized Algorithms for Cut and Cycle Hitting Problems on H-Minor-Free Graphs

We design the first subexponential-time (parameterized) algorithms for several cut and cycle-hitting problems on $H$-minor free graphs. In particular, we obtain the following results (where $k$ is the solution-size parameter). 1. $2^{O(\sqrt{k}\log k)} \cdot n^{O(1)}$ time algorithms for Edge Bipartization and Odd Cycle Transversal; 2. a $2^{O(\sqrt{k}\log^4 k)} \cdot n^{O(1)}$ time algorithm for Edge Multiway Cut and a $2^{O(r \sqrt{k} \log k)} \cdot n^{O(1)}$ time algorithm for Vertex Multiway Cut, where $r$ is the number of terminals to be separated; 3. a $2^{O((r+\sqrt{k})\log^4 (rk))} \cdot n^{O(1)}$ time algorithm for Edge Multicut and a $2^{O((\sqrt{rk}+r) \log (rk))} \cdot n^{O(1)}$ time algorithm for Vertex Multicut, where $r$ is the number of terminal pairs to be separated; 4. a $2^{O(\sqrt{k} \log g \log^4 k)} \cdot n^{O(1)}$ time algorithm for Group Feedback Edge Set and a $2^{O(g \sqrt{k}\log(gk))} \cdot n^{O(1)}$ time algorithm for Group Feedback Vertex Set, where $g$ is the size of the group. 5. In addition, our approach also gives $n^{O(\sqrt{k})}$ time algorithms for all above problems with the exception of $n^{O(r+\sqrt{k})}$ time for Edge/Vertex Multicut and $(ng)^{O(\sqrt{k})}$ time for Group Feedback Edge/Vertex Set. We obtain our results by giving a new decomposition theorem on graphs of bounded genus, or more generally, an $h$-almost-embeddable graph for any fixed constant $h$. In particular we show the following. Let $G$ be an $h$-almost-embeddable graph for a constant $h$. Then for every $p\in\mathbb{N}$, there exist disjoint sets $Z_1,\dots,Z_p \subseteq V(G)$ such that for every $i \in \{1,\dots,p\}$ and every $Z'\subseteq Z_i$, the treewidth of $G/(Z_i\backslash Z')$ is $O(p+|Z'|)$. Here $G/(Z_i\backslash Z')$ is the graph obtained from $G$ by contracting edges with both endpoints in $Z_i \backslash Z'$.

==> Saket/applications.tex <==
In this section, we apply our framework of Section \ref{sec:framework} on several problems to obtain sub-exponential algorithms on $H$-minor free graphs. Given the framework, its application on a problem is fairly straightforward, except we have to ensure that the problem satisfies the requirements of this framework. First, we apply this framework on \probOCT and describe all the steps in detail. For other problems, the applications are similar. Thus, for convenience, we will just describe the changes needed for those problems omitting the trivial details. In all of our problems, we assume that the input graph is $H$-minor-free. 

\subsection{\probOCT and \probEB}
First, we consider the  \probOCT (OCT) problem. In OCT, we are given a graph $G=(V,E)$ and a parameter $k$, and we would like to decide whether there is a subset $V'\subseteq V$ of size at most $k$ such that for each odd cycle $C$ in $G$, there is a vertex of $C$ that is in $V'$. If there is such a subset, we refer to it as a solution. By abusing the notation, we refer to a solution to the OCT problem also as an OCT. The distinction should be clear from the context. Following our framework, the first step is to apply Lemma~\ref{lem-candidate} to obtain a candidate set $\mathsf{Cand} \subseteq V$ for the instance. Note that this takes only a polynomial time. For our purpose, it is sufficient to find a solution which is a subset of $\mathsf{Cand}$. Henceforth, by the term solution we always mean a subset of $\mathsf{Cand}$.       

Note that after removing the vertices in an OCT from $G$, a bipartite graph is left. For such a bipartition, we arbitrarily define the left and the right side (or partition). Consider any subgraph $G_1=(V_1,E_1)$ and fix any solution to OCT on $G_1$. We define a configuration $\lambda$ of $V'\subseteq V_1$ w.r.t. the solution to be a set of values corresponding to the vertices  in $V'$, where each value is in $\{1,2,3\}$. We note that these three values denote whether the corresponding vertex $v$ is in the solution, is in the left side of the residual bipartite graph (after removing the solution OCT) or is in the right side of the residual bipartite graph. As we want our solution to be a subset of $\mathsf{Cand}$, the 1-vertices must always come from $\mathsf{Cand}$. Otherwise, we say the configuration is not valid. 

\subsubsection{Contraction-friendly Tree-decomposition DP} 

First, we describe the desired contraction-friendly tree-decomposition DP for OCT. We are given an $n$-vertex graph $G=(V,E)$, a (possibly empty) subset $X\subseteq V$, and a tree-decomposition $\mathcal{T}$ of $G/X$. Let $T$ be the underlying tree of $\mathcal{T}$. For any $0\le l\le k$, we would like to decide whether there is a solution to OCT on $G$ of size $l$ which is disjoint from $X$. In particular, we would like to use the tree-decomposition $\mathcal{T}$ to solve this problem efficiently. For that purpose, first we define a subproblem on each vertex $t\in T$. As the bag $\beta(t)$ of $t$ might contain contracted vertices, we have to be careful in defining the subproblem. 

To define the subproblem, we need the following definition. For each subset $V'$ of vertices in $G/X$, let ${(G/X)(V')}^{-1}$ be the subgraph of $G$ that is the pre-image of ${(G/X)}[V']$, i.e., ${(G/X)(V')}^{-1}$ is obtained by undoing the contractions of all vertices in the induced subgraph ${(G/X)}[V']$. 
%Similarly, define ${(G/X)}^{-1}(\sigma(t))$. 

\begin{observation}\label{obs:distinct-config}
The number of distinct configurations of the vertices in ${(G/X)(V')}^{-1}$ w.r.t. the solutions disjoint from $X$ is $2^{O(|V'|)}$. 
\end{observation} 

\begin{proof}
%Consider any solution $S$ of OCT disjoint from $X$ on any graph $G'$ that contains ${(G/X)}^{-1}(\sigma(t))$ as an induced subgraph. 
For each contracted vertex $v$ of $V'$, consider the connected component $C$ in $G[X]$ corresponding to $v$. Then as the solutions we seek are disjoint from $X$, $C$ must be bipartite. Hence, the number of distinct configuration of the vertices in $C$ w.r.t. such  solutions is only 2 depending on which partition is designated as the left or right. Also, any vertex $u$ of $V'\backslash X$ can have 3 configurations. Hence, the number of such distinct configurations of the vertices in ${(G/X)(V')}^{-1}$ is at most $3^{|V'|}=2^{O(|V'|)}$.  
\end{proof}

Note that given ${(G/X)(V')}^{-1}$, one can easily compute the $2^{O(|V'|)}$ such configurations. For any solution $S$ and a configuration $\lambda$ of a set of vertices $V'$, we say $S$ is consistent with $\lambda$ if the 1-vertices of $V'$ are in $S$, and 2- and 3-vertices of $V'$ are in the left and right side of the residual bipartite graph. For any configuration $\lambda$ of the vertices in ${(G/X)(\sigma(t))}^{-1}$ and $0\le l\le k$, we define a subproblem where the goal is to decide whether there is a solution to OCT on ${(G/X)(\gamma(t))}^{-1}$ which is disjoint from $X$, is consistent  with $\lambda$ and uses exactly $\ell$ vertices of ${(G/X)(\gamma(t)\backslash \sigma(t))}^{-1}$. Thus, in this subproblem, the solution contains 1-vertices of $\sigma(t)$ and $\ell$ additional vertices from ${(G/X)(\gamma(t)\backslash \sigma(t))}^{-1}$. We store the boolean value (YES/NO) of the solution of this subproblem in a table $L(t)$ indexed by $(\lambda,l)$. For simplicity, we assume wlog that all configurations are valid, i.e., for each configuration $\lambda$, 1-vertices of ${(G/X)(\sigma(t))}^{-1}$ come from $\mathsf{Cand}$. By Observation \ref{obs:distinct-config}, the number of entries that we need to store in $L(t)$ is $2^{O(|\sigma(t)|)}\cdot k$, and all such relevant configurations can be computed in $2^{O(|\sigma(t)|)}n^{O(1)}$ time. 

For our application, we cannot assume that the treewidth of $T$ is bounded. Instead, we make two assumptions: (i) the bag size of each non-leaf vertex in $T$ is bounded by a parameter $w$, and (ii) for each leaf $t\in T$, the table $L(t)$ is given to us. With these assumptions, we show that the table entries corresponding to all vertices of $T$ can be computed in time $2^{O(w)}n^{O(1)}$. 

Consider any non-leaf vertex $t\in T$. We can assume that the tables corresponding to the children of $t$ are already computed. Fix any configuration $\lambda$ of the vertices in ${(G/X)(\sigma(t))}^{-1}$ and an integer $0\le l\le k$. We want to compute the entry in $L(t)$ w.r.t. $(\lambda,l)$. First, we guess a configuration $\lambda'$ of the vertices in ${(G/X)(\beta(t)\backslash \sigma(t))}^{-1}$ w.r.t. the solutions disjoint from $X$. Thus, we have the configuration of all vertices in $\beta(t)$. This gives us the configuration $\lambda(s)$ of $\sigma(s)$ for each child $s$ of $t$. We note that the vertices of $\beta(t)$ might be shared by multiple children. But, in our subproblems, the solution size does not account for the vertices in the adhesion. Thus, these solutions account for disjoint sets of vertices, and hence the subproblems can be treated as independent. Let $\ell^u$ be the number of 1-vertices in $\beta(t)\backslash \sigma(t)$ w.r.t. $\lambda'$. Then, we would like to compute a solution, which consists of these 1-vertices and $\ell_s$ vertices from ${(G/X)(\gamma(s)\backslash \sigma(s))}^{-1}$ for each child $s$ of $t$, where $\ell=\ell^u+\sum_s \ell_s$. Using the tables of the children, we can easily compute such a solution if possible, and hence the entry $(\lambda,l)$ can be computed in polynomial time. Now, as we need to enumerate all possible $2^{O(|\beta(t)\backslash \sigma(t)|)}$ configurations $\lambda'$, it is not hard to see that computation of each entry takes $2^{O(|\beta(t)\backslash \sigma(t)|)}n^{O(1)}$ time. Hence, the table for $t$ can be computed in time $2^{O(|\beta(t)|)}n^{O(1)}=2^{O(w)}n^{O(1)}$.  
     

% \begin{lemma}\label{lem:contraction-friendly}
% Suppose we are given a graph $G=(V,E)$, a (possibly empty) subset $X\subseteq V$, a subset $\mathsf{Cand}\subseteq V$, a tree-decomposition $\mathcal{T}$ of $G/X$ of width $w$, and an integer $\tau$, such that $G$ has a solution to OCT contained in $\mathsf{Cand}$ and of size $\tau$ that is disjoint from $X$. Then a solution to OCT on $G$ contained in $\mathsf{Cand}$, disjoint from $X$ and of size $\tau$ can be obtained in time $2^{O(w)}n^{O(1)}$.   
% \end{lemma}

\subsubsection{The Algorithm}
Now, we describe our main algorithm. First, we apply Lemma \ref{lem-rsdecomp} to compute in polynomial time a tree decomposition $\mathcal{T}_\textnormal{RS}$ of $G$ with adhesion size at most $h$ in which the torso of each vertex is $h$-almost-embeddable. Note that $h$ is a constant which depends only on $H$. Given $\mathcal{T}_\textnormal{RS}$, the idea is to employ a DP on it to solve OCT on $G$. However, we have to be careful here, as the width of $\mathcal{T}_\textnormal{RS}$ can be very large. Next, we describe our DP based algorithm to solve OCT on $\mathcal{T}_\textnormal{RS}$. 

Let ${T}_\textnormal{RS}$ be the underlying tree of $\mathcal{T}_\textnormal{RS}$. The DP algorithm stores a table $M(t)$ for each vertex $t \in {T}_\textnormal{RS}$. 
%We define a configuration $\lambda$ of $\sigma(t)$ to be a set of values corresponding to the vertices  in $\sigma(t)$, where each value is in $\{1,2,3\}$. We note that these three values denote whether the corresponding vertex $v$ is in the solution, is in the left side of the residual bipartite graph (after removing the solution OCT) or is in the right side of the residual bipartite graph. As we want our solution to be a subset of $\mathsf{Cand}$, the 1-vertices must always come from $\mathsf{Cand}$. Otherwise, we say the configuration is not valid. 
Each entry of $M(t)$ is indexed by a tuple $(\lambda,l)$ for a configuration $\lambda$ of $\sigma(t)$ and an integer $0\le l\le k$ which stores a boolean value YES/NO based on whether or not there is an OCT for $G[\gamma(t)]$ such that the OCT is consistent with $\lambda$ and uses exactly $\ell$ vertices of $\gamma(t)\backslash \sigma(t)$.
%, i.e., 1-vertices of $\sigma(t)$ are in the OCT, and 2- and 3-vertices of $\sigma(t)$ are in the left and right side of the residual bipartite graph. 
That is, the entry w.r.t. $(\lambda,l)$ stores the solution of the problem $\mathsf{Prob}_{\lambda,l}$ as defined in our framework. Note that the size of the table $M(t)$ is $O(k)$, as $\sigma(t)$ is at most the constant $h$. Next, we show how to compute the entries of $M(t)$. 

%In the base case, we compute the entries corresponding to the leaves of $\mathcal{T}_\textnormal{RS}$. Consider any such leaf $t$. Note that, by definition, $G[\beta(t)]$ itself is the torso of $t$, and hence is $h$-almost-embeddable. Fix any configuration $\lambda$ of $\sigma(t)$ and an integer $0\le l\le k$. We would like to compute the entry of $M(t)$ w.r.t. $(\lambda,l)$. The $l=0$ case is trivial. So, assume $l \ge 1$. If the entry w.r.t. $(\lambda,l-1)$ is YES, we can readily say the entry w.r.t. $(\lambda,l)$ is also YES. So, let us consider the other case. In this case, we apply Lemma~\ref{lem-key} on the graph $G[\beta(t)\backslash \gamma(t)]$ with $p = \lfloor \sqrt{k} \rfloor$ to obtain the disjoint sets $Z_1,\dots,Z_p$. Following the framework, for each $Z'$ that is a subset of some $Z_i\cap \mathsf{Cand}$, of size $O(k/p)=O(\sqrt{k})$, we solve OCT on the graph $G[\beta(t)]$ assuming the desired solution is disjoint from $Z_i\backslash Z'$. That is, we need to solve $\mathsf{Prob}_{\lambda,l,Z_i \backslash Z'}$. To do this, first we use the observation that $\mathbf{tw}(G[\beta(t)\backslash \gamma(t)]/(Z_i \backslash Z')) = O(p+|Z'|)=O(\sqrt{k})$, and compute a tree-decomposition $\mathcal{T}$ of $G[\beta(t)\backslash \gamma(t)]/(Z_i \backslash Z')$ of width $O(\sqrt{k})$. Note that we also want our solution to be consistent with the configuration $\lambda$. We know the 1-vertices $\sigma_1(t)\subseteq \sigma(t)$ are already selected in the solution. So, we just consider the subset $\sigma'(t)= \sigma(t)\backslash \sigma_1(t)$ and contract the connected components in $G[\sigma'(t)]$. Thereafter we add these contracted vertices to all bags of $\mathcal{T}$. Note that the treewidth of $\mathcal{T}$ still remains $O(\sqrt{k})$. Moreover, $\mathcal{T}$ is a tree-decomposition of $G[\beta(t)\backslash \sigma_1(t)]/X$ where $X=(Z_i \backslash Z')\cup \sigma'(t)$. Note that we need to compute an OCT of size at most $l$ in $G[\beta(t)\backslash \sigma_1(t)]$ such that the vertices in $(Z_i \backslash Z')\cup \sigma'(t)$ are disjoint from the desired solution. Hence, we apply Lemma \ref{lem:contraction-friendly} on $G[\beta(t)\backslash \sigma_1(t)]$ with $X$ and $\mathcal{T}$ as defined above, and $\tau=l$. If the algorithm in the lemma computes a valid solution, we set our entry $(\lambda,l)$ to YES and go to the next entry. Otherwise, we probe the next set $Z'$. Note that there can be $k^{O(\sqrt{k})}$ such set $Z'$ and the algorithm in Lemma \ref{lem:contraction-friendly} uses $2^{O(\sqrt{k})}n^{O(1)}$ time. Thus, computation of an entry $(\lambda,l)$ requires $k^{O(\sqrt{k})}n^{O(1)}$ time. It follows that the table of a leaf $t$ can be computed in the same time bound.       

%Let ${T}_\textnormal{RS}$ be the underlying tree of $\mathcal{T}_\textnormal{RS}$. 
Consider any vertex $t\in {T}_\textnormal{RS}$.   %Also fix a configuration $\lambda$ of $\sigma(t)$ and $1\le l\le k$. Again assume that the entry w.r.t. $(\lambda,l-1)$ stores NO. 
We can assume that the table entries corresponding to the children (if any) of $t$ are already computed. This is true, as in the base case, we deal with the leaves of ${T}_\textnormal{RS}$. First, we apply Corollary~\ref{cor-extention} on $t$ with $p = \lfloor \sqrt{k} \rfloor$ to obtain the sets $Y_1,\dots,Y_p \subseteq \gamma(t) \backslash \sigma(t)$. Then, following the framework, we construct the set $\varPi$ of pairs $(i,Y')$, where $i \in [p]$ and $Y' \subseteq Y_i$, satisfying three conditions: \textbf{(1)} $|\varPi| = |\mathsf{Cand}|^{O(\sqrt{k})}$, \textbf{(2)} $|Y'| = O(k/p)$ for all $(i,Y') \in \varPi$, and \textbf{(3)} for any configuration $\lambda$ of $\sigma(t)$ and $0\le l\le k$, the answer to $\mathsf{Prob}_{\lambda,l}$ is YES iff the answer to $\mathsf{Prob}_{\lambda,l,Y_i \backslash Y'}$ is YES for some $(i,Y') \in \varPi$. Thus, we can focus on a fixed set $Y'\subseteq Y_i$ and solve $\mathsf{Prob}_{\lambda,l,Y_i \backslash Y'}$ for all $\lambda$ and $l$. Again, following the framework, we apply Lemma \ref{lem-specialtd} to obtain a tree-decomposition $\mathcal{T}^*$ of $G[\gamma(t)]/(Y_i \backslash Y')$ in time $2^{O(\sqrt{k})} n^{O(1)}$. Any non-leaf vertex in the underlying tree ${T}^*$ of $\mathcal{T}^*$ has bag size $O(\sqrt{k})$. However, for a leaf, the bag size can be large. Nevertheless, by Property \textbf{(iii)} in Lemma \ref{lem-specialtd}, for such a leaf $t^* \in {T}^*$, $\gamma(t^*) = \beta(t^*) = \gamma(s)$ and $\sigma(t^*) = \sigma(s)$ for some $s \in C_i$. Recall that $C_i$ is the set of children $s$ of $t$ satisfying $\gamma(s) \cap Y_i = \emptyset$. Thus, by our assumption, the table $M(t^*)$ corresponding to $t^*$ is already computed. Subsequently, we apply the contraction-friendly DP on the tree-decomposition $\mathcal{T}^*$. 
%, and $\tau=l$. Note that Lemma \ref{lem:contraction-friendly} demands a tree-decomposition of bounded width, which $\mathcal{T}^*$ does not have. However, using the observation above regarding leaves of $T^*$, one can trivially adapt the proof of Lemma \ref{lem:contraction-friendly} to handle this special case. 
Now, by Property \textbf{(ii)} in Lemma \ref{lem-specialtd}, the root $\mathsf{rt}$ of $T^*$ has only one child $\mathsf{rt}'$, where $\sigma(\mathsf{rt}') = \sigma(t)$ and $ \beta(\mathsf{rt}) = \sigma(t)$. Also, note that $\sigma(t)\cap Y_i=\emptyset$, and so $\sigma(t)\cap (Y_i \backslash Y')=\emptyset$. Thus, the vertices of $\sigma(t)$ are not contracted in  $\mathcal{T}^*$. Hence, 
%$\beta(\mathsf{rt}) = \sigma(t)$, where  $\mathsf{rt}$ is the root of $T^*$. 
the table $L(\mathsf{rt}')$ computed by the contraction-friendly DP contains entries corresponding to all possible configurations of $\sigma(\mathsf{rt}') = \sigma(t)$ and all $0\le l\le k$. Thus, this is exactly the table needed for $t$, and  we can just set $M(t)[\lambda,l]\leftarrow M(t)[\lambda,l] \lor L(\mathsf{rt}')[\lambda,l]$ for each configuration $\lambda$ of $\sigma(t)$ and $0\le l\le k$. Note that in our solutions, we do not count the vertices of $\sigma(t)$. But, this can be easily fixed at the end by adding the  1-vertices for each configuration to the computed solution and computing the best combined solution.   

Now, the contraction-friendly DP takes $2^{O(w)}n^{O(1)}$ time, where $w$ is the bag size of any non-leaf vertex in $T^*$. Also, the total number of pairs $(i,Y')$ in $\varPi$ is ${|\textsf{Cand}|}^{O(\sqrt{k})}n^{O(1)}$. Thus, the computation of $M(t)$ takes in total $|\textsf{Cand}|^{O(\sqrt{k})}\cdot 2^{O(w)}\cdot n^{O(1)}$ time. As the bag size of any non-leaf vertex in ${T}^*$ is $O(\sqrt{k})$, a trivial upper bound on this is $n^{O(\sqrt{k})}$. Also, by Lemma \ref{lem-candidate}, the size of $\textsf{Cand}$ for OCT is $k^{O(1)}$. Subsequently, we obtain the time bound of $2^{O(\sqrt{k}\log k)}n^{O(1)}$. It follows that the OCT problem on $G$ can be solved in the same time bound. 

\begin{theorem}
\probOCT on $H$-minor free graphs can be solved in $2^{O(\sqrt{k}\log k)}n^{O(1)}$ time. 
\end{theorem}

\subsubsection{\probEB}
The \probEB (EB) problem is similar to OCT, except here we need to remove a subset of edges. Formally, we are given an $H$-minor-free graph $G=(V,E)$ and a parameter $k$, and we would like to decide whether there is a subset $E'\subseteq E$ of size at most $k$ such that removal of the edges in $E'$ from $G$ gives us a bipartite graph. As we saw in the previous subsection, the main ingredient for applying the framework is the contraction-friendly tree-decomposition DP. Here, we describe such a DP for EB. The rest of the algorithm is similar to the one for OCT. 

% If there is such a subset, we refer to it as a solution. By abusing the notation, we refer to a solution to the OCT problem also as an OCT. The distinction should be clear from the context. Following our framework, the first step is to apply Lemma~\ref{lem-candidate} to obtain a candidate set $\mathsf{Cand} \subseteq V$ of size $k^{O(1)}$ for the instance. Note that this takes only a polynomial time. For our purpose, it is sufficient to find a solution which is a subset of $\mathsf{Cand}$. Henceforth, by the term solution we always mean a subset of $\mathsf{Cand}$.       

Consider any subgraph $G_1=(V_1,E_1)$ and fix any solution $E_\mathsf{sol}$ on $G_1$. We say that $E_\mathsf{sol}$ is disjoint from a set of vertices $X$ if the endpoints of the edges in $E_\mathsf{sol}$ are disjoint from $X$. We define a configuration $\lambda$ of $V'\subseteq V_1$ w.r.t. the solution to be a set of values corresponding to the vertices  in $V'$, where each value is in $\{1,2\}$. We note that these values denote whether the corresponding vertex $v$ is in the left side of the residual bipartite graph (after removing the solution edges) or is in the right side of the residual bipartite graph. Next, we describe the contraction-friendly tree-decomposition DP for EB.  

We are given an $n$-vertex graph $G=(V,E)$, a (possibly empty) subset $X\subseteq V$, and a tree-decomposition $\mathcal{T}$ of $G/X$. Let $T$ be the underlying tree of $\mathcal{T}$. For any $0\le l\le k$, we would like to decide whether there is a solution to EB on $G$ of size $l$ which is disjoint from $X$. The following observation is similar to Observation \ref{obs:distinct-config}. 

\begin{observation}\label{obs:distinct-config-EB}
The number of distinct configurations of the vertices in ${(G/X)(V')}^{-1}$ w.r.t. the solutions disjoint from $X$ is $2^{O(|V'|)}$. 
\end{observation} 

For any solution $S$ and a configuration $\lambda$ of a set of vertices $V'$, we say $S$ is consistent with $\lambda$ if the 1- and 2-vertices of $V'$ are in the left and right side of the residual bipartite graph. For any configuration $\lambda$ of the vertices in ${(G/X)(\sigma(t))}^{-1}$ and $0\le l\le k$, we define a subproblem where the goal is to decide whether there is a solution to EB on ${(G/X)(\gamma(t))}^{-1}$ which is disjoint from $X$, consistent with $\lambda$ and uses exactly $\ell$ edges such that at least one endpoint of each edge is not in ${(G/X)(\sigma(t))}^{-1}$. Thus, in this subproblem, the solution contains the edges whose both endpoints are 1-vertices (or 2-vertices) among the set of edges $E^1$ in ${(G/X)(\sigma(t))}^{-1}$ and $\ell$ additional edges from ${(G/X)(\gamma(t))}^{-1}$ which are not in $E^1$. We store the boolean value (YES/NO) of the solution of this subproblem in a table $L(t)$ indexed by $(\lambda,l)$. 

We note that it is sufficient to solve the above subproblem, as the edges used in a solution from ${(G/X)(\sigma(t))}^{-1}$ can be easily derived from the corresponding configuration. The subproblem is defined in this way to avoid any potential multiple counting of a solution edge at different levels. In this setting, if an edge $(u,v)$ is common to both parent and child subproblems, the decision to take it or not is uniquely determined by the configuration corresponding to the children. 

By Observation \ref{obs:distinct-config-EB}, the number of entries that we need to store in $L(t)$ is $2^{O(|\sigma(t)|)}\cdot k$, and all such relevant configurations can be computed in $2^{O(|\sigma(t)|)}n^{O(1)}$ time. With these modified definitions of subproblem and DP table, the rest of the algorithm is similar to  the one for OCT. Hence, we conclude that the table entries corresponding to all vertices of $T$ can be computed in time $2^{O(w)}n^{O(1)}$, where $w$ is the maximum size of the bags of the non-leaf vertices in $T$. 

Note that by our framework, the total running time of our algorithm is $(|\textsf{Cand}|^{O(\sqrt{k})}\cdot 2^{O(w)})\cdot n^{O(1)}$, where $w=\sqrt{k}$. By Lemma \ref{lem-candidate}, the size of $\textsf{Cand}$ for EB is $k^{O(1)}$. Subsequently, we obtain the time bound of $2^{O(\sqrt{k}\log k)}n^{O(1)}$.  

\begin{theorem}
\probEB on $H$-minor free graphs can be solved in $2^{O(\sqrt{k}\log k)}n^{O(1)}$ time. 
\end{theorem}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



\subsection{\probGFVS and \probGFES}
For a directed graph $G=(V,A)$, a finite group $\Sigma$ of size $g$ and a labeling function $\Lambda: A\rightarrow \Sigma$, $(G,\Lambda)$ is called a $\Sigma$-labeled graph if for each arc $(u,v)\in A$, $(v,u)$ is also in $A$ and $\Lambda((u,v))=\Lambda((v,u))^{-1}$. For a subset of vertices $D$, we denote by $(G\backslash D,\Lambda)$ the $\Sigma$-graph obtained by removing the vertices in $D$ from $(G,\Lambda)$. Similarly, for a subset of arcs $A'$, we denote by $(G\backslash A',\Lambda)$ the $\Sigma$-labeled graph obtained by removing the arcs in $A'$ from $(G,\Lambda)$. For a cycle $C=\{v_1,\ldots,v_t,v_1\}$, let $\Lambda(C)=\Lambda((v_1,v_2))\cdot \ldots \cdot \Lambda((v_{t-1},v_t))\cdot \Lambda((v_t,v_1))$. Here $\cdot $ is the group operation. A cycle $C$ is called a non-null cycle if $\Lambda(C)\ne 1_{\Sigma}$. In the \probGFVS (GFVS) problem, given a $\Sigma$-labeled graph $(G,\Lambda)$ and a parameter $k$, the goal is to decide whether there is a set of vertices $D$ such that $(G\backslash D,\Lambda)$ does not have any non-null cycle. The \probGFES (GFES) problem is similar, except here the goal is to decide whether there is a set of arcs $A'$ such that $(G\backslash A',\Lambda)$ does not have any non-null cycle. For simplicity, we assume that $\Sigma=\{1,\ldots,g\}$.  

First, we apply our framework on GFVS. We note that OCT is a specialization of GFVS when $\Sigma=\{0,1\}$ \cite{KratschW20}. Indeed, our algorithm for GFVS is an extension of the algorithm for OCT. In the following, we just describe the contraction-friendly tree-decomposition DP for GFVS. The remaining algorithm is similar to the one for OCT. Following our framework, the first step is to obtain a candidate set $\mathsf{Cand} \subseteq V$. Henceforth, by the term solution we always mean a subset of $\mathsf{Cand}$.       

For describing our algorithm, we need a definition. For a $\Sigma$-labeled graph $(G,\Lambda)$, $\mu: V\rightarrow \Sigma$ is called a consistent labeling iff for each arc $(u,v)$ in $G$, we have $\mu(v)=\mu(u)\cdot \Lambda((u,v))$. 

\begin{lemma}\label{lem:consistentlabels}
\cite{Guillemot11a} A $\Sigma$-labeled graph has a consistent labeling iff it does not contain any non-null cycle. 
\end{lemma}

Consider any subgraph $G_1=(V_1,A_1)$ and fix any solution $S$ of GFVS on $G_1$. Also, consider a consistent labeling $\mu$ of the vertices in the graph $(G\backslash D,\Lambda)$, which exists by the above lemma. We define a configuration $\lambda$ of $V'\subseteq V_1$ w.r.t. $S$ to be a set of values corresponding to the vertices in $V'$, where each value is in $\{0,1,\ldots,g\}$. We note that these values denote whether the corresponding vertex $v$ is in the solution (0) or is mapped to the element $i\in \Sigma$ via $\mu$. As we want our solution to be a subset of $\mathsf{Cand}$, the 0-vertices must always come from $\mathsf{Cand}$. We also say that $S$ is \emph{compatible} with the configuration $\lambda$.  


\begin{observation}\label{obs:distinct-config-gfvs}
The number of distinct configurations of the vertices in ${(G/X)(V')}^{-1}$ w.r.t. the solutions disjoint from $X$ is $g^{O(|V'|)}$. 
\end{observation} 

\begin{proof}
%Consider any solution $S$ of OCT disjoint from $X$ on any graph $G'$ that contains ${(G/X)}^{-1}(\sigma(t))$ as an induced subgraph. 
For each contracted vertex $v$ of $V'$, consider the connected component $C$ in $G[X]$ corresponding to $v$. Then as the solutions we seek are disjoint from $X$, $C$ must have no non-null cycles. It follows that the vertices of $C$ has a consistent labeling $\mu$. Now, fix the label of any vertex in $C$. By definition of consistent labeling, this also fixes the labeling of the remaining vertices of $C$. Thus, the number of distinct labelings of the vertices of $C$ is only $g$. Hence, the number of distinct configurations of the vertices in $C$ w.r.t. the solutions disjoint from $X$ is only $g$. Also, any vertex $u$ of $V'\backslash X$ can have $g+1$ configurations. Hence, the number of such distinct configurations of the vertices in ${(G/X)(V')}^{-1}$ is at most $(g+1)^{|V'|}=g^{O(|V'|)}$.  
\end{proof}

Next, we describe the contraction-friendly tree-decomposition DP for GFVS. A subproblem is defined in the same way as for OCT. For any configuration $\lambda$ of the vertices in ${(G/X)(\sigma(t))}^{-1}$ and $0\le l\le k$, we define a subproblem where the goal is to decide whether there is a solution to GFVS on ${(G/X)(\gamma(t))}^{-1}$ which is disjoint from $X$, is compatible with $\lambda$ and  uses exactly $\ell$ vertices of ${(G/X)(\gamma(t)\backslash \sigma(t))}^{-1}$. We store the boolean value (YES/NO) of the solution of this subproblem in a table $L(t)$ indexed by $(\lambda,l)$. For simplicity, we assume wlog that all configurations are valid, i.e., for each configuration $\lambda$, 1-vertices of ${(G/X)(\sigma(t))}^{-1}$ come from $\mathsf{Cand}$. 
By Observation \ref{obs:distinct-config-gfvs}, the number of entries that we need to store in $L(t)$ is $g^{O(|\sigma(t)|)}\cdot k$, and all such relevant configurations can be computed in $g^{O(|\sigma(t)|)}n^{O(1)}$ time. With these modified definitions of subproblem and DP table, the rest of the algorithm is similar to  the one for OCT. Hence, we conclude that the table entries corresponding to all vertices of $T$ can be computed in time $g^{O(w)}n^{O(1)}$, where $w$ is the maximum size of the bags of the non-leaf vertices in $T$. 

Note that by our framework, the total running time of our algorithm is $(|\textsf{Cand}|^{O(\sqrt{k})}\cdot g^{O(w)})\cdot n^{O(1)}$, where $w=\sqrt{k}$. A trivial upper bound on this is $(ng)^{O(\sqrt{k})}$. Also, by Lemma \ref{lem-candidate}, the size of $\textsf{Cand}$ for GFVS is $k^{O(g)}$. Subsequently, we obtain the time bound of $2^{O(g \sqrt{k}\log(gk))} \cdot n^{O(1)}$.  

\begin{theorem}
\probGFVS on $H$-minor free graphs can be solved in $\min\{(ng)^{O(\sqrt{k})},$ $2^{O(g \sqrt{k}\log(gk))} \cdot n^{O(1)}\}$ time. 
\end{theorem}


\subsubsection{\probGFES}
The algorithm for GFES is similar to the one for GFVS. Here, we describe the main differences. For simplicity, we use the terms edge and arc interchangeably. Consider any subgraph $G_1=(V_1,E_1)$ and fix any solution $E_\mathsf{sol}$ on $G_1$. We say that $E_\mathsf{sol}$ is disjoint from a set of vertices $X$ if the endpoints of the edges in $E_\mathsf{sol}$ are disjoint from $X$. Consider a consistent labeling $\mu$ of the vertices in the graph $(G\backslash E_\mathsf{sol},\Lambda)$, which exists by Lemma \ref{lem:consistentlabels}. We define a configuration $\lambda$ of $V'\subseteq V_1$ w.r.t. $E_\mathsf{sol}$ to be a set of values corresponding to the vertices in $V'$, where each value is in $\{1,\ldots,g\}$. We note that these values denote whether the corresponding vertex $v$ is mapped to the element $i\in \Sigma$ via $\mu$. We also say that $S$ is \emph{compatible} with the configuration $\lambda$. The following observation is similar to Observation \ref{obs:distinct-config-gfvs}.  


\begin{observation}\label{obs:distinct-config-gfes}
The number of distinct configurations of the vertices in ${(G/X)(V')}^{-1}$ w.r.t. the solutions disjoint from $X$ is $g^{O(|V'|)}$. 
\end{observation} 

Next, we describe the contraction-friendly tree-decomposition DP for GFES. For any configuration $\lambda$ of the vertices in ${(G/X)(\sigma(t))}^{-1}$ and $0\le l\le k$, we define a subproblem where the goal is to decide whether there is a solution to GFES on ${(G/X)(\gamma(t))}^{-1}$ which is disjoint from $X$, consistent with $\lambda$ and uses exactly $\ell$ edges such that at least one endpoint of each edge is not in ${(G/X)(\sigma(t))}^{-1}$. We store the boolean value (YES/NO) of the solution of this subproblem in a table $L(t)$ indexed by $(\lambda,l)$. By Observation \ref{obs:distinct-config-gfes}, the number of entries that we need to store in $L(t)$ is $g^{O(|\sigma(t)|)}\cdot k$, and all such relevant configurations can be computed in $g^{O(|\sigma(t)|)}n^{O(1)}$ time. With these modified definitions of subproblem and DP table, the rest of the algorithm is similar to  the one for EB. Hence, we conclude that the table entries corresponding to all vertices of $T$ can be computed in time $g^{O(w)}n^{O(1)}$, where $w$ is the maximum size of the bags of the non-leaf vertices in $T$. 

Note that by our framework, the total running time of our algorithm is $(|\textsf{Cand}|^{O(\sqrt{k})}\cdot g^{O(w)})\cdot n^{O(1)}$, where $w=\sqrt{k}$. A trivial upper bound on this is $(ng)^{O(\sqrt{k})}$. Also, by Lemma \ref{lem-candidate}, the size of $\textsf{Cand}$ for GFES is $k^{O(\log^3 k)}$. Subsequently, we obtain the time bound of $2^{O(\sqrt{k} \log g \log^4 k)} \cdot n^{O(1)}$.  

\begin{theorem}
\probGFES on $H$-minor free graphs can be solved in $\min\{(ng)^{O(\sqrt{k})},$ $2^{O(\sqrt{k} \log g \log^4 k)} \cdot n^{O(1)}\}$ time. 
\end{theorem}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    

\subsection{\probVMultiC and \probEMultiC}
In \probVMultiC (VMC), given a graph $G=(V,E)$, a collection $U$ of $r$ pairs of vertices $U \subseteq V \times V$, and an integer $k$, the goal is to decide if there is a set of $k$ vertices of $V \backslash R$ whose removal separates each pair of vertices in $U$ where $R$ is the set of vertices appearing in the pairs of $U$. \probEMultiC (EMC) is similar, except here we remove a set of $k$ edges. Here $R$ is called the set of terminals. First, we consider VMC. Following our framework, the first step is to obtain a candidate set $\mathsf{Cand} \subseteq V$. Henceforth, by the term solution we always mean a subset of $\mathsf{Cand}$. Next, we describe the contraction-friendly tree-decomposition DP for VMC. Our DP is a natural extension of a DP for bounded treewidth graphs \cite{GuoHKNU08}. 

We are given an $n$-vertex graph $G=(V,E)$, a (possibly empty) subset $X\subseteq V$, and a tree-decomposition $\mathcal{T}$ of $G/X$. Let $T$ be the underlying tree of $\mathcal{T}$. We would like to solve a subproblem in ${(G/X)(\gamma(t))}^{-1}$. Consider any partition $\Pi$ of $R$ such that each pair in $U$ appears in two different parts. We can have $|R|^{O(|R|)}=r^{O(r)}$ such distinct partitions. Note that each such partition helps us guess which terminals will be on the same connected component after removal of a solution. We  define subproblems with respect to $\Pi$, assuming $\Pi$ is the correct configuration of the terminals. Let $\alpha\le 2r$ be the number of parts. We treat each part as a color between $1$ to $\alpha$. 

Consider any subgraph $G_1=(V_1,E_1)$ and fix any solution $S$ on $G_1$. We define a configuration $\lambda$ of $V'\subseteq V_1$ w.r.t. the solution to be a set of values corresponding to the vertices in $V'$, where each value is in $\{0,1,2,\ldots,\alpha\}$. We note that these values denote whether the corresponding vertex $v$ is in $S$ (0), or is in the $i$-th connected component along with the vertices of $R$ in $i$-th part ($i$). We say that $S$ is consistent with $\lambda$.  

\begin{observation}\label{obs:distinct-config-vmc}
The number of distinct configurations of the vertices in ${(G/X)(V')}^{-1}$ w.r.t. the solutions disjoint from $X$ is ${\alpha}^{O(|V'|)}$. 
\end{observation} 

\begin{proof}
%Consider any solution $S$ of OCT disjoint from $X$ on any graph $G'$ that contains ${(G/X)}^{-1}(\sigma(t))$ as an induced subgraph. 
For each contracted vertex $v$ of $V'$, consider the connected component $C$ in $G[X]$ corresponding to $v$. Then as the solutions we seek are disjoint from $X$, all vertices in $X$ have the same value in any configuration w.r.t. such a solution. Hence, the number of distinct configurations of the vertices in $C$ w.r.t. such  solutions is only $\alpha$ depending on the connected component in which they end up. Also, any vertex $u$ of $V'\backslash X$ can have at most $\alpha+1$ configurations. Hence, the number of such distinct configurations of the vertices in ${(G/X)(V')}^{-1}$ is at most ${(\alpha+1)}^{|V'|}={\alpha}^{O(|V'|)}$.  
\end{proof}

For any configuration $\lambda$ of the vertices in ${(G/X)(\sigma(t))}^{-1}$ and $0\le l\le k$, we define a subproblem where the goal is to decide whether there is a solution to VMC on ${(G/X)(\gamma(t))}^{-1}$ which is disjoint from $X$, is consistent  with $\lambda$ and uses exactly $\ell$ vertices of ${(G/X)(\gamma(t)\backslash \sigma(t))}^{-1}$. We store the boolean value (YES/NO) of the solution of this subproblem in a table $L(t)$ indexed by $(\lambda,l)$. By Observation \ref{obs:distinct-config-vmc}, the number of entries that we need to store in $L(t)$ is $r^{O(|\sigma(t)|)}\cdot k$, and all such relevant configurations can be computed in $r^{O(|\sigma(t)|)}n^{O(1)}$ time. With these modified definitions of subproblem and DP table, the rest of the algorithm is similar to  the one in \cite{GuoHKNU08}. Hence, we conclude that the table entries corresponding to all vertices of $T$ can be computed in time $r^{O(r+w)}n^{O(1)}$, where $w$ is the maximum size of the bags of the non-leaf vertices in $T$. 

Note that by our framework, the total running time of our algorithm is $(|\textsf{Cand}|^{O(\sqrt{k})}\cdot r^{O(r+w)})\cdot n^{O(1)}$, where $w=\sqrt{k}$. A trivial upper bound on this is $n^{O(\sqrt{k}+r)}$, as $r\le n^2$. Also, by Lemma \ref{lem-candidate}, the size of $\textsf{Cand}$ for VMC is $k^{O(\sqrt{r})}$. Subsequently, we obtain the time bound of $2^{O(r\sqrt{k} \log k)} \cdot n^{O(1)}$.  

\begin{theorem}
\probVMultiC on $H$-minor free graphs can be solved in 
$\min\{n^{O(\sqrt{k}+r)}, 
2^{O((\sqrt{rk}+r) \log rk))} \cdot n^{O(1)}
\}$ 
time. 
\end{theorem}


As mentioned in \cite{GuoHKNU08}, the DP for VMC is almost the same as the DP for EMC. Similarly, the contraction-friendly tree-decomposition DP for EMC is very similar to the one for VMC. Also, the candidate set size for EMC is $(r+k)^{O(\log^3(r+k))}$. Hence, we obtain the following theorem. 

\begin{theorem}
\probEMultiC on $H$-minor free graphs can be solved in 
$\min\{n^{O(\sqrt{k}+r)}, 
2^{O((r+\sqrt{k})\log^4 (rk))} \cdot n^{O(1)}
\}$ 
time.
\end{theorem}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\subsection{\probVMC and \probEMC}
In \probVMC (VMWC), given a graph $G$, a subset of $r$ vertices $R \subseteq V (G)$, called terminals, and an integer $k$, the goal is to decide if there is a set of at most $k$ vertices of $V(G) \backslash R$ hitting every path between a pair of terminals. \probEMC (EMWC) is similar, except the goal is to decide if there is a set of at most $k$ edges of $E(G)$ hitting every path between a pair of terminals. 

Note that VMWC is a special case of VMC where we have to separate all $r^2$ pairs of terminals in $R\times R$. Also, we need to consider only one partition where each terminal belongs to a separate part. Thus, we readily obtain a contraction free DP that runs in $r^{O(w)}n^{O(1)}$ time.  

By our framework, the total running time of our algorithm is $(|\textsf{Cand}|^{O(\sqrt{k})}\cdot r^{O(w)})\cdot n^{O(1)}$, where $w=\sqrt{k}$. A trivial upper bound on this is $n^{O(\sqrt{k})}$, as $r\le n$. Also, by Lemma \ref{lem-candidate}, the size of $\textsf{Cand}$ for VMWC is $k^{O(r)}$. Subsequently, we obtain the time bound of $2^{O(r\sqrt{k} \log k)} \cdot n^{O(1)}$.  

\begin{theorem}
\probVMC on $H$-minor free graphs can be solved in $\min\{n^{O(\sqrt{k})},$ $2^{O(r\sqrt{k} \log k)} \cdot n^{O(1)}\}$ time. 
\end{theorem}

\subsection{\probEMC}
We describe the contraction-friendly tree-decomposition DP for EMWC. This DP is partly motivated by the DP in \cite{DengLZ13} for Multi-Multiway cut which is a generalization of EMWC. We are given an $n$-vertex graph $G=(V,E)$, a (possibly empty) subset $X\subseteq V$, and a tree-decomposition $\mathcal{T}$ of $G/X$. Let $T$ be the underlying tree of $\mathcal{T}$. Consider any non-leaf vertex $t \in T$. Note that removal of the solution edges in EMWC induces a partition of the vertices where each part (or connected component) contains at most one terminal of $R$. We would like to guess an optimal partition. Consider any subset $V' \subseteq \beta(t)$, and any partition $\Pi=\{X_i\mid i\in I\}$ of the vertices in ${(G/X)(V')}^{-1}$ for some index set $I$. We say a set of edges $C$ in ${(G/X)(\gamma(t))}^{-1}$ is consistent with $\Pi$ and vice versa iff 
\begin{itemize}
    \item The endpoints of the edges in $C$ are disjoint from $X$;
    \item $C$ separates all the terminals; and
    \item Let $G'$ be the subgraph ${(G/X)(\gamma(t))}^{-1}$ after removing the edges in $C$. Let $\{P_i\mid i\in I\}$ be the family of connected components such that $P_i\cap V'\ne \emptyset$ for all $i\in I$. Then $X_i=P_i$ for all $i\in I$. 
\end{itemize}

\begin{observation}\label{obs:distinct-config-emwc}
The number of distinct partitions of the vertices in ${(G/X)(V')}^{-1}$ consistent with sets of edges is ${|V'|}^{O(|V'|)}$.
\end{observation} 

\begin{proof}
%Consider any solution $S$ of OCT disjoint from $X$ on any graph $G'$ that contains ${(G/X)}^{-1}(\sigma(t))$ as an induced subgraph. 
First note that the number of distinct partitions of the vertices in $V'$ is ${|V'|}^{O(|V'|)}$. However, $(G/X)$ $(V'){}^{-1}$ might contain many more vertices, as we undo the contraction of the component vertices in $V'$. For each contracted vertex $v$ of $V'$, consider the connected component $C$ in $G[X]$ corresponding to $v$. Then as the endpoints of the edges in consistent sets $C$ are disjoint from $X$, all vertices in $X$ must end up in the same connected component after removal of the edges from $C$. It follows that the number of such distinct partitions of the vertices in ${(G/X)(V')}^{-1}$ is again bounded by ${|V'|}^{O(|V'|)}$. 
\end{proof}

For any partition $\Pi$ of the vertices in ${(G/X)(\sigma(t))}^{-1}$, we define a subproblem where the goal is to find the minimum size set of edges $C$ in ${(G/X)(\gamma(t))}^{-1}$ which is consistent with $\Pi$. It is sufficient to solve this subproblem for our purpose, as if we know the minimum value, we can also solve the decision version of the problem. We store a solution $C$ of this subproblem in a table $L(t)$ indexed by $\Pi$. To compute the table corresponding to $t$, we need to merge the tables of its children. In the following, we describe how to merge the tables of two children. One can easily extend it to more than two children.  

Consider any partition $\Pi_1$ of the vertices in ${(G/X)(\sigma(t))}^{-1}$. We extend this partition to obtain a partition $\Pi_2$ of the vertices in ${(G/X)(\beta(t))}^{-1}$. For the purpose of extension, we define compatibility of two partitions. Consider two partitions  $\Pi_1=\{X_i\mid i\in I\}$ and $\Pi_2=\{Y_j\mid j\in J\}$. Also, consider the bipartite graph $B=(I,J,E')$ such that $(i,j)\in E'$ iff $X_i\cap Y_j\ne \emptyset$. Then $\Pi_1$ and $\Pi_2$ are compatible if $E'$ is a perfect matching and for each edge $(i,j)\in E'$, $i=j$. 
%Consider such a mergeable pair. For $(i,i)\in E'$, let $Z_i=(X_i\cup Y_i)\cap \beta(t)$. Let $\Pi=\cup_i Z_i$. We denote $\Pi$ by $\Pi_1\xor \Pi_2$. 

Now, fix a partition $\Pi$ of the vertices in ${(G/X)(\sigma(t))}^{-1}$. We show how to compute the entry $L(t)[\Pi]$ by merging tables of two children $s_1$ and $s_2$. First, we take a partition $\Pi'$ of the vertices in ${(G/X)(\beta(t))}^{-1}$ which is compatible with $\Pi$. Given $\Pi'$, the partition of the vertices in  ${(G/X)(\sigma(s_1))}^{-1}$ (or ${(G/X)(\sigma(s_2))}^{-1}$) compatible with $\Pi'$, is also fixed. Let $\Pi_1$ and $\Pi_2$ be these two partitions w.r.t. $s_1$ and $s_2$. The entry $L(t)[\Pi]=\arg \min_{|C|} \{C=L(s_1)[\Pi_1]\cup L(s_2)[\Pi_2]\cup C'\}$, where $C'$ is a subset of edges $\{(u,v)\mid u,v \notin X\}$ such that $(u,v)$ is in ${(G/X)(\beta(t))}^{-1}$, but not in ${(G/X)(\gamma(s_1))}^{-1}$ or ${(G/X)(\gamma(s_2))}^{-1}$, and $u$ and $v$ are contained in different parts of $\Pi'$.   

The correctness follows from the fact that if an edge $(u,v)$ is common to both parent and child subproblems, the decision to take it or not is uniquely determined by the partition corresponding to the children. Thus, no edge is counted more than once in the computed solution.  

Note that computation of a table entry requires enumerating all possible $\Pi'$. The number of such partitions is bounded by $w^{O(w)}$ by Observation \ref{obs:distinct-config-emwc}, where $w$ is the maximum size of the bags of the non-leaf vertices in $T$. By the same observation, the number of entries that we need to store in $L(t)$ is ${|\sigma(t)|}^{O(|\sigma(t)|)}\cdot k$, and all such relevant partitions can be computed in ${|\sigma(t)|}^{O(|\sigma(t)|)}n^{O(1)}$ time. Hence, we conclude that the table entries corresponding to all vertices of $T$ can be computed in time $w^{O(w)} n^{O(1)}$. 

By our framework, the total running time of our algorithm is $(|\textsf{Cand}|^{O(\sqrt{k})}\cdot w^{O(w)})\cdot n^{O(1)}$, where $w=\sqrt{k}$. A trivial upper bound on this is $n^{O(\sqrt{k})}$. Also, by Lemma \ref{lem-candidate}, the size of $\textsf{Cand}$ for EMWC is $k^{O(\log^3 k)}$. Subsequently, we obtain the time bound of $2^{O(\sqrt{k}\log^4 k)} \cdot n^{O(1)}$.  

\begin{theorem}
\probEMC on $H$-minor free graphs can be solved in $2^{O(\sqrt{k}\log^4 k)} \cdot n^{O(1)}$ time. 
\end{theorem}


==> Saket/saketPreamble.tex <==
%\usepackage{microtype}%if unwanted, comment out or use option "draft"
\usepackage{wrapfig}
\usepackage{bm}

\usepackage{graphicx,color}
\usepackage{empheq}
\usepackage{tcolorbox}
\definecolor{blueish}{rgb}{0.122, 0.435, 0.698}
\definecolor{dagstuhlyellow}{rgb}{0.99,0.78,0.07}
\definecolor{lightgray}{rgb}{0.9,0.9,0.9}
\newtcbox{\colbox}{
size=title,
  nobeforeafter,
  colframe=white,
  colback=blue!5!white,
  arc=10pt,
  tcbox raise base}
  
  
  
\newcommand{\defparproblemR}[4]{
  \vspace{1mm}
\noindent\colbox{
  \begin{minipage}{0.94\textwidth}
  \begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}lr} #1  &
    {\textbf{Parameter:}} #3 \\ \end{tabular*}
  {\textbf{Input:}} #2  \\
  {\textbf{Task:}} #4
  \end{minipage}
  }
 % \vspace{1mm}
}

%\newcommand{\defparproblemRNP}[4]{
% % \vspace{1mm}
%  \begin{center}
%\noindent\colbox{
%  \begin{minipage}{0.44\textwidth}
%  \begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}lr} #1  \end{tabular*}
%  {\textbf{Input:}} #2  \\
%  {\textbf{Task:}} #3
%  \end{minipage}
%  }
%\end{center}
% % \vspace{1mm}
%}




\newcommand{\defparproblemRNP}[3]{
  \begin{center}
\noindent\colbox{
  \begin{minipage}{0.85\textwidth}
\begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}lr} #1  \end{tabular*}
  {\textbf{Input:}} #2  \\
  {\textbf{Task:}} #3
  \end{minipage}
  }
\end{center}
}


\usepackage{xspace}
\newcommand{\pname}{\textsc}
\newcommand{\ProblemFormat}[1]{\pname{#1}}
\newcommand{\ProblemIndex}[1]{\index{problem!\ProblemFormat{#1}}}
\newcommand{\ProblemName}[1]{\ProblemFormat{#1}\ProblemIndex{#1}{}\xspace}

\newcommand{\probPVD}{\ProblemName{Planar Vertex Deletion}}
\newcommand{\probCVD}{\ProblemName{Chordal Vertex Deletion}}
\newcommand{\probEB}{\ProblemName{Edge Bipartization}}
\newcommand{\probOCT}{\ProblemName{Odd Cycle Transversal}}
\newcommand{\probEMC}{\ProblemName{Edge Multiway Cut}}
\newcommand{\probVMC}{\ProblemName{Vertex Multiway Cut}}
\newcommand{\probVrMC}{\ProblemName{Vertex $r$-Multiway Cut}}
\newcommand{\probGFVS}{\ProblemName{Group Feedback Vertex Set}}
\newcommand{\probGFES}{\ProblemName{Group Feedback Edge Set}}
\newcommand{\probGFEVS}{\ProblemName{Group Feedback Edge/Vertex Set}}
\newcommand{\probEMultiC}{\ProblemName{Edge Multicut}}
\newcommand{\probErMultiC}{\ProblemName{Edge $r$-Multicut}}
\newcommand{\probVMultiC}{\ProblemName{Vertex Multicut}}
\newcommand{\probVrMultiC}{\ProblemName{Vertex $r$-Multicut}}
\newcommand{\probEVMultiC}{\ProblemName{Edge/Vertex Multicut}}
\newcommand{\probSFVS}{\ProblemName{Subset Feedback Vertex Set}}

\newcommand{\probTWdel}{\ProblemName{Treewidth-$\eta$ Modulator}}
\newcommand{\probFdel}{\ProblemName{$\mathcal{F}$-Deletion}}
\newcommand{\probFpack}{\ProblemName{$\mathcal{F}$-Packing}}
\newcommand{\probSdel}{\ProblemName{$\mathcal{S}$-Deletion}}
\newcommand{\probSpack}{\ProblemName{$\mathcal{S}$-Packing}}
% Commonly used names
\newcommand{\probVC}{\ProblemName{Vertex Cover}}
\newcommand{\probPlVC}{\ProblemName{Planar Vertex Cover}}
\newcommand{\probPVC}{\ProblemName{Partial Vertex Cover}}
\newcommand{\probPDS}{\ProblemName{Partial Dominating Set}}
\newcommand{\probPrDS}{\ProblemName{Partial $r$-Dominating Set}}
\newcommand{\probFVS}{\ProblemName{Feedback Vertex Set}}
\newcommand{\probIFVS}{\ProblemName{Independent Feedback Vertex Set}}
\newcommand{\probCycPacking}{\ProblemName{Cycle Packing}}
\newcommand{\probPlFVS}{\ProblemName{Planar Feedback Vertex Set}}
\newcommand{\probIS}{\ProblemName{Independent Set}}
\newcommand{\probWIS}{\ProblemName{Weighted Independent Set}}
\newcommand{\probMCIS}{\ProblemName{Multicolored Independent Set}}
\newcommand{\probDS}{\ProblemName{Dominating Set}}
\newcommand{\probrDS}{\ProblemName{$r$-Dominating Set}}
\newcommand{\probrSC}{\ProblemName{$r$-Scattered Set}}
%\newcommand{\probMDS}{\ProblemName{Minimum Dominating Set}}
\newcommand{\probPlDS}{\ProblemName{Planar Dominating Set}}
\newcommand{\probCDS}{\ProblemName{Connected Dominating Set}}
\newcommand{\probDST}{\ProblemName{Dominating Set on Tournaments}}
\newcommand{\probClique}{\ProblemName{Clique}}
\newcommand{\probMC}{\ProblemName{Multicolored Clique}}
\newcommand{\probPClique}{\ProblemName{Partitioned Clique}}
\newcommand{\probqSC}{\ProblemName{$q$-Set Cover}}
\newcommand{\probSC}{\ProblemName{Set Cover}}
\newcommand{\probDSP}{\ProblemName{Dominating Set with Pattern}}
%\newcommand{\probOCT}{\ProblemName{Odd Cycle Transversal}}
%\newcommand{\probEB}{\ProblemName{Edge Bipartization}}
\newcommand{\probHam}{\ProblemName{Hamiltonian Cycle}}
\newcommand{\probPlHam}{\ProblemName{Planar Hamiltonian Cycle}}
\newcommand{\probHamP}{\ProblemName{Hamiltonian Path}}
\newcommand{\probKPath}{\ProblemName{Longest Path}}
\newcommand{\probWKPath}{\ProblemName{Weighted Longest Path}}
\newcommand{\probthreeSAT}{\ProblemName{$3$-SAT}}
\newcommand{\probqSAT}{\ProblemName{$q$-SAT}}
\newcommand{\probcnfSAT}{\ProblemName{CNF-SAT}}
\newcommand{\probthreeCol}{\ProblemName{$3$-Coloring}}
\newcommand{\probqCol}{\ProblemName{$q$-Coloring}}
\newcommand{\probListColoring}{\ProblemName{List Coloring}}
\newcommand{\probOddSet}{\ProblemName{Odd Set}}
\newcommand{\probTuring}{\ProblemName{Short Turing Machine Acceptance}}
\newcommand{\probSI}{\ProblemName{Subgraph Isomorphism}}
\newcommand{\probGI}{\ProblemName{Graph Isomorphism}}
\newcommand{\probWCS}{\ProblemName{Weighted Circuit Satisfiability}}
\newcommand{\probClosestString}{\ProblemName{Closest String}}
\newcommand{\probClosestSubstring}{\ProblemName{Closest Substring}}
\newcommand{\probGridTiling}{\ProblemName{Grid Tiling}}
\newcommand{\probGridTilingLeq}{\ProblemName{Grid Tiling with~$\le$}}
\newcommand{\probUnitDisk}{\ProblemName{Unit Disk Independent Set}}
\newcommand{\probEMWay}{\ProblemName{Edge Multiway Cut}}
\newcommand{\probEDS}{\ProblemName{Edge Dominating Set}}
\newcommand{\probEMWaySets}{\ProblemName{Edge Multiway Cut for Sets}}
\newcommand{\probDirEMWay}{\ProblemName{Directed Edge Multiway Cut}}
\newcommand{\probEMCut}{\ProblemName{Edge Multicut}}
\newcommand{\probMulticut}{\ProblemName{Multicut}}
\newcommand{\probDirEMCut}{\ProblemName{Directed Edge Multicut}}
\newcommand{\probSkewEMCut}{\ProblemName{Skew Edge Multicut}}
\newcommand{\probDFVS}{\ProblemName{Directed Feedback Vertex Set}}
\newcommand{\probDFAS}{\ProblemName{Directed Feedback Arc Set}}
\newcommand{\probDFASC}{\ProblemName{Directed Feedback Arc Set Compression}}
\newcommand{\probPartpq}{\ProblemName{$(p,q)$-Partition}}
\newcommand{\probClusterpq}{\ProblemName{$(p,q)$-Cluster}}
\newcommand{\probSatellite}{\ProblemName{Satellite Problem}}
\newcommand{\probTw}{\ProblemName{Treewidth}}
\newcommand{\probPerfSetMatch}{\ProblemName{Perfect $d$-Set Matching}}
\newcommand{\probHS}{\ProblemName{Hitting Set}}
\newcommand{\probdHS}{\ProblemName{$d$-Hitting Set}}
\newcommand{\probEdHS}{\ProblemName{E$d$-Hitting Set}}
\newcommand{\probSetSplit}{\ProblemName{Set Splitting}}
\newcommand{\probSteiner}{\ProblemName{Steiner Tree}}
\newcommand{\probSteinerF}{\ProblemName{Steiner Forest}}
\newcommand{\probMotif}{\ProblemName{Graph Motif}}
\newcommand{\probColorfulMotif}{\ProblemName{Colorful Graph Motif}}
\newcommand{\probRBDSlong}{\ProblemName{Red-Blue Dominating Set}}
\newcommand{\probRBDS}{\ProblemNameX{RBDS}{Red-Blue Dominating Set}}
\newcommand{\probCRBDSlong}{\ProblemName{Colored Red-Blue Dominating Set}}
\newcommand{\probCRBDS}{\ProblemNameX{Col-RBDS}{Colored Red-Blue Dominating Set}}
\newcommand{\probCVC}{\ProblemName{Connected Vertex Cover}}
\newcommand{\probCFVS}{\ProblemName{Connected Feedback Vertex Set}}
\newcommand{\probCBullHit}{\ProblemName{Connected Bull Hitting}}
\newcommand{\probSetPacking}{\ProblemName{Set Packing}}
\newcommand{\probDisFactors}{\ProblemName{Disjoint Factors}}
\newcommand{\probDisPaths}{\ProblemName{Vertex Disjoint Paths}}
\newcommand{\probChromatic}{\ProblemName{Chromatic Number}}
\newcommand{\probECC}{\ProblemName{Edge Clique Cover}}
\newcommand{\probSubsetSum}{\ProblemName{Subset Sum}}
\newcommand{\probKnapsack}{\ProblemName{Knapsack}}
\newcommand{\probWayCut}{\ProblemName{$s$-Way Cut}}
\newcommand{\probEulerian}{\ProblemName{Eulerian  Deletion}}
\newcommand{\probBisec}{\ProblemName{Minimum Bisection}}
\newcommand{\probMaxBisec}{\ProblemName{Maximum Bisection}}


==> Saket/useless <==
\section{OCT in $H$-minor-free graphs}

Before describing our algorithm, we first introduce a generalization of the OCT problem, called \textit{constrained OCT}.

\begin{definition}
For a graph $G = (V,E)$ and a triple $(V_0,V_1,V_2)$ of subsets of $V$, we say an odd cycle transversal $V_\mathsf{oct}$ of $G$ is $(V_0,V_1,V_2)$-\textbf{compatible} if \textbf{(i)} $V_0 \subseteq V_\mathsf{oct}$ and \textbf{(ii)} $V_1 \backslash V_\mathsf{oct}$ and $V_2 \backslash V_\mathsf{oct}$ belong to different parts in the bipartite graph $G-V_\mathsf{oct}$.
\end{definition}
\begin{definition}[constrained OCT]
The \textbf{constrained OCT} problem is a parameterized problem in which each instance is a 5-tuple $(G,V_0,V_1,V_2,k)$ where $G$ is a graph, $V_0,V_1,V_2$ are three disjoint subsets of $V(G)$, and $k \in \mathbb{N}$ is the parameter, and the goal is to decide whether $G$ has an odd cycle transversal $V_\mathsf{oct}$ of size at most $k$ that $(V_0,V_1,V_2)$-compatible.
%\textbf{(i)} $V_0 \subseteq V_\mathsf{oct}$, $V_1 \subseteq I_1$, $V_2 \subseteq I_2$, \\
%\textbf{(ii)} $I_1$ and $I_2$ are independent sets in $G$, \\
%\textbf{(iii)} $|V_\mathsf{oct}| \leq k$.
\end{definition}

%Our main technical contribution is the following lemma, which plays an important role in our OCT algorithm for $H$-minor-free graphs.

%The proof of Lemma~\ref{lem-structure} will be given in Section~\ref{sec-proofstr}.
%Before this, let us first describe our OCT algorithm, assuming Lemma~\ref{lem-structure} holds.
Our OCT algorithm is obtained by (nontrivially) combining the ideas of Robertson-Seymour decomposition, recursive understanding, Baker's technique, and a technical lemma we establish about the structure of a graph that admits a good star decomposition (Lemma~\ref{lem-structure}).
Let $G$ be the input graph, which is $H$-minor-free.
Let $h > 0$ be the constant in Lemma~\ref{lem-rsdecomp} and $h'$ be the smallest integer that is larger than $|V(\mathsf{rep}(\mathcal{C}))|$ for any equivalence class $\mathcal{C}$ of $\equiv_\mathsf{oct}$ in $\mathcal{F}_{\subseteq [h]}$.

\paragraph{High-level framework.}
Algorithm~\ref{alg-OCT} presents the high-level framework of our algorithm.
The algorithm consists of an initialization step (Line~1), the main loop (Line~2-12), and a finalization step (Line~13).
In the initialization step, we compute an $(h,h')$-good tree decomposition $(T,\beta)$ for $G$ with adhesion size at most $h$ (together with the almost-embeddable structure of the torso of each internal node of $T$).
To this end, we first compute the Robertson-Seymour decomposition $(T_0,\beta)$ for $G$ (Lemma~\ref{lem-rsdecomp}), which has adhersion size at most $h$ and $h$-almost-embeddable torsos.
Then for each leaf $t \in T_0$, we add to $t$ a child $t'$ with bag $\beta(t') = \emptyset$; let $T$ be the resulting tree.
It is clear that $(T,\beta)$ is a tree decomposition of $G$ with adhesion size at most $h$.
Note that each leaf of $T$ has an empty bag and each internal node of $T$ is a node of $T_0$ (hence its torso is $h$-almost-embeddable).
So $(T,\beta)$ is $(h,0)$-good and thus an $(h,h')$-good.

The main loop (Line~2-12) is the heart of our algorithm.
Roughly speaking, during the loop, what we do is to iteratively \textit{simplify} the problem instance $(G,k)$.
That is, in each iteration, we generate a new instance $(G,k)$ from the old one such that the new instance is a YES-instance iff the old one is.
Meanwhile, we maintain the tree decomposition $(T,\beta)$ to guarantee that it is always an $(h,h')$-good tree decomposition of the current graph $G$ with adhesion size $h$.
A detailed discussion of the main loop will be given shortly.
Before this, we first discuss when the loop terminates and what we do in the finalization step.

We terminate the main loop when the problem instance $(G,k)$ becomes ``sufficiently simple'' in the sense that $|T| = 1$, i.e., the tree $T$ has only a root node (Line~2).
At this point, we reach the finalization step (Line~13), which simply solves the instance $(G,k)$ by \textit{brute-force}.
Why are we able to use brute-force when $|T| = 1$?
As mentioned before, $(T,\beta)$ is always an $(h,h')$-good tree decomposition of $G$.
When $|T|=1$, the bag $\beta(t)$ of the only node $t \in T$ is of size at most $h'$, because $t$ is a leaf and $(T,\beta)$ is $(h,h')$-good.
It follows that $G$ consists of a subgraph $G_0$ with $|V(G_0)| \leq h'$ and some isolated vertices.
Therefore, $(G,k)$ is a YES-instance iff $(G_0,k)$ is.
Since $|V(G_0)| \leq h'$, the instance $(G_0,k)$ can be solved in constant time by brute-force.

\begin{algorithm}[h]
    \caption{\textsc{OddCycleTransversal}$(G,k)$}
	\begin{algorithmic}[1]
        \State Compute an $(h,h')$-good tree decomposition $(T,\beta)$ of $G$ with adheresion size at most $h$
        %\State \textsc{Contract}$((T,\beta),h')$
        \While{$|T| \geq 2$}
            \State $t \leftarrow$ an internal node of $T$ whose children are all leaves
            %\State $X \leftarrow \gamma(t)$ and $B \leftarrow \sigma(t)$
            \State $\mathcal{I}_\mathsf{yes} \leftarrow \emptyset$
            \For{all $V_0,V_1,V_2 \subseteq \sigma(t)$ and all $l \in [k+h]$}
                \State Solve the constrained OCT instance $(G[\gamma(t)],V_0,V_1,V_2,l)$
                \If{$(G[\gamma(t)],V_0,V_1,V_2,l)$ is a YES-instance}
                    \State $\mathcal{I}_\mathsf{yes} \leftarrow \mathcal{I}_\mathsf{yes} \cup \{(G[\gamma(t)],V_0,V_1,V_2,l)\}$
                \EndIf
            \EndFor
            \If{$(G[\gamma(t)],\emptyset,\emptyset,\emptyset,k) \notin \mathcal{I}_\mathsf{yes}$}
                \textbf{return} NO
            \EndIf
            %\State $\lambda \leftarrow$ an arbitrary bijection from $\sigma(t)$ to $[|\sigma(t)|]$
            %\State view both $G[\gamma(t)]$ and $G[\gamma'(t)]$ as boundaried graphs in $\mathcal{F}_{[|\sigma(t)|]}$
            \State $(G^*,c) \leftarrow$ \textsc{Representative}$(G[\gamma(t)],\mathcal{I}_\mathsf{yes})$
            \State $G \leftarrow G^* \oplus G[\gamma'(t)]$ and $k \leftarrow k-c$
            \State Modify $(T,\beta)$ by replacing the subtree $T_t$ with a single node $t^*$ with $\beta(t^*) = V(G^*)$
            %\State \textsc{Contract}$((T,\beta),h')$
        \EndWhile
        \State Solve the instance $(G,k)$ by brute-force
        %\nolinenumbers
	\end{algorithmic}
	\label{alg-OCT}
\end{algorithm}

In what follows, we discuss the main loop in detail.
In each iteration of the loop, we first pick an (arbitrary) internal node $t \in T$ whose children are all leaves (Line~3).
Note that the subtree $T_t$ is a star.
Consider the induced subgraph $G[\gamma(t)]$.
Fix a bijection $\lambda: \sigma(t) \rightarrow [|\sigma(t)|]$.
We can view $G[\gamma(t)]$ as a boundaried graph in $\mathcal{F}_{[|\sigma(t)|]}$ with boundary $\sigma(t)$ and labeling $\lambda$.
%Similarly, the labeling $\lambda$ also makes $G[\gamma'(t)]$ a boundaried graph in $\mathcal{F}_{[|\sigma(t)|]}$, and we have $G = G[\gamma(t)] \oplus G[\gamma'(t)]$.
Our goal in this iteration is to compute a progressive representative of the equivalent class of $\equiv_\mathsf{oct}$ containing $G[\gamma(t)]$.
To this end, the critical step is to solve a set of constrained OCT instances on $G[\gamma(t)]$ (Line~5-8).
Specifically, we solve the instances $(G[\gamma(t)],V_0,V_1,V_2,l)$ for all $V_0,V_1,V_2 \subseteq \sigma(t)$ and all $l \in [k+h]$.
This is the most technical part of our algorithm, and the main idea is to exploit the fact that $G[\gamma(t)]$ has a $(h,h')$-good \textit{star} decomposition, which is $(T_t,\beta)$.
We shall establish a structural lemma (Lemma~\ref{lem-structure}) for graphs that admit a good star decomposition, which then allows us to apply Baker's technique and dynamic programming on tree decomposition to solve the problem.
After the constrained OCT instances are solved, we then include the YES-instances (Line~8) in $\mathcal{I}_\mathsf{yes}$.
If $(G[\gamma(t)],\emptyset,\emptyset,\emptyset,k) \notin \mathcal{I}_\mathsf{yes}$, then we can immediately conclude that $(G,k)$ is a NO-instance (Line~9), because $(G[\gamma(t)],k)$ is a NO-instance.
Otherwise, we use the information of $\mathcal{I}_\mathsf{yes}$ to compute a progressive representative of the equivalent class of $\equiv_\mathsf{oct}$ containing $G[\gamma(t)]$ and the corresponding transposition (Line~10).
Specifically, the sub-routine \textsc{Representative} takes $G[\gamma(t)]$ and $\mathcal{I}_\mathsf{yes}$ as input, and output a pair $(G^*,c)$ where $G^*$ is a progressive representative of the equivalent class containing $G[\gamma(t)]$ and $c \in \mathbb{Z}^+$ is the transposition from $G[\gamma(t)]$ to $G'$.
Note that $G = G[\gamma(t)] \oplus G[\gamma'(t)]$, if we regard $G[\gamma'(t)]$ as a boundaried graph with boundary $\sigma(t)$ and labeling $\lambda$.
Thus, by the definition of a progressive representative, we know that $(G,k)$ is a YES-instance of OCT iff $(G^* \oplus G[\gamma'(t)],k-c)$ is.
We then replace $(G,k)$ with $(G^* \oplus G[\gamma'(t)],k-c)$ (Line~11).
After this, we modify the tree decomposition $(T,\beta)$ by replacing the subtree $T_t$ with a single node $t^*$ with $\beta(t^*) = V(G^*)$ (Line~12).
It is easy to see that after the modification, $(T,\beta)$ is a tree decomposition of the new $G$, i.e., $G^* \oplus G[\gamma'(t)]$, which is still $(h,h')$-good and with adhesion size at most $h$.
Furthermore, $|T|$ strictly decreases after the modification.
Therefore, the loop will terminate in at most $m$ iterations, where $m$ is the initial size of $T$.
This directly implies the correctness of our algorithm.
Next, we discuss the only two missing pieces of our algorithm, which are \textbf{(1)} how to solve the instances on $G[\gamma(t)]$ (Line~6) and \textbf{(2)} how to compute the progressive representative $G^*$ and the transposition $c$ (Line~10).

\paragraph{Solving the instances on $G[\gamma(t)]$.}
Consider a constrained OCT instance $(G[\gamma(t)],V_0,V_1,V_2,l)$ where $V_0,V_1,V_2 \subseteq \sigma(t)$ and $l \in [k+h]$.
We want to test if there exists a $(V_0,V_1,V_2)$-compatible OCT of $G[\gamma(t)]$ of size at most $l$.
If $l < |V_0|$, then $(G[\gamma(t)],V_0,V_1,V_2,l)$ is clearly a NO-instance.
So assume $l \geq |V_0|$.
First, we notice that using Lemma~\ref{lem-candidate}, we are able to compute a small relevant set for the instance.
\begin{corollary} \label{cor-candidate}
We can compute in $|\gamma(t)|^{O(1)}$ time a set $S \subseteq \gamma(t)$ of size $l^{O(1)}$ such that with probability at least $1-1/2^{|\gamma(t)|}$, $G[\gamma(t)]$ has a $(V_0,V_1,V_2)$-compatible OCT of size $l$ iff $G$ has a $(V_0,V_1,V_2)$-compatible OCT of size $l$ that is contained in $S$.
\end{corollary}
\begin{proof}
Let $G'$ be the graph obtained from $G[\gamma(t)] - V_0$ by adding edges $(u,v)$ for all $u \in V_1 \backslash V_0$ and $v \in V_2 \backslash V_0$.
One can easily verify that a subset $U \subseteq V(G')$ is an OCT of $G'$ iff $U \cup V_0$ is a $(V_0,V_1,V_2)$-compatible OCT of $G[\gamma(t)]$.
Furthermore, every $(V_0,V_1,V_2)$-compatible OCT of $G[\gamma(t)]$ can be written as $U \cup V_0$ where $U$ is an OCT of $G'$.
In other words, the map $U \mapsto U \cup V_0$ gives a one-to-one correspondence between the OCTs of $G'$ and the $(V_0,V_1,V_2)$-compatible OCTs of $G[\gamma(t)]$.
Therefore, if we use the algorithm of Lemma~\ref{lem-candidate} to compute a set $S' \subseteq V(G')$ of size $(l-|V_0|)^{O(1)}$ such that $G'$ has an OCT of size $l-|V_0|$ iff $G'$ has an OCT of size $l-|V_0|$ that is contained in $S'$, then the set $S = S' \cup V_0$ satisfies the property that $G[\gamma(t)]$ has a $(V_0,V_1,V_2)$-compatible OCT of size $l$ iff $G$ has a $(V_0,V_1,V_2)$-compatible OCT of size $l$ that is contained in $S$.
\end{proof}

Let $S \subseteq \gamma(t)$ be the set in the above corollary.
As mentioned before, we shall exploit the fact that $G[\gamma(t)]$ has an $(h,h')$-good star decomposition with adhesion size $h$.
To this end, we establish the following technical lemma, whose proof is deferred to Section~\ref{sec-proofstr}.

\begin{lemma} \label{lem-structure}
Let $G$ be a graph admitting a $(c,c')$-good star decomposition with adhesion size $c''$ for some constants $c,c',c''$.
Then for any $p \in [n]$, there are $Z_1,\dots,Z_p \subseteq V(G)$ satisfying the following. \\
\textbf{(i)} Each vertex $v \in V(G)$ is contained in at most $c''$ sets in $\{Z_1,\dots,Z_p\}$. \\
\textbf{(ii)} For any $i \in [p]$ and $V' \subseteq Z_i$, $\mathbf{tw}(G/(Z_i-V')) = O(p+|V'|)$, where the constant hidden in the big-$O$ notation depends on $c,c',c''$. \\
%one can compute in $|V(G)|^{O(1)}$ time a tree decomposition of $G \backslash V'$ in which each bag contains $O(p)$ vertices in $V(G) \backslash V_i$ and intersects $O(p')$ connected component of $G[V_i \backslash V']$ where $p' = |V'|$. \\
Furthermore, if the good star decomposition of $G$ (and the almost-embeddable structure of the torso of the central bag) is given, then the above sets $Z_1,\dots,Z_p$ can be computed in $|V(G)|^{O(1)}$ time.
\end{lemma}

We apply the above lemma with $G = G[\gamma(t)]$ and $p = \lfloor\sqrt{l}\rfloor$, and obtain the sets $Z_1,\dots,Z_p \subseteq V(G[\gamma(t)]) = \gamma(t)$.
We claim that $G[\gamma(t)]$ has a $(V_0,V_1,V_2)$-compatible OCT of size at most $l$ iff for some $i \in [p]$ and $V' \subseteq Z_i \cap S$ with $|V'| \leq hl/p$, $G[\gamma(t)]$ has a $(V_0,V_1,V_2)$-compatible OCT of size at most $l$ that is \textit{disjoint} with $Z_i - V'$.
The ``if'' part is obvious.
To see the ``only if'' part, assume $G[\gamma(t)]$ has a $(V_0,V_1,V_2)$-compatible OCT of size at most $l$.
Then it has a $(V_0,V_1,V_2)$-compatible OCT $V_\mathsf{oct} \subseteq S$ of size at most $l$ by Corollary~\ref{cor-candidate}.
By the property \textbf{(i)} in Lemma~\ref{lem-structure}, each vertex $v \in \gamma(t)$ is contained in at most $h$ sets in $\{Z_1,\dots,Z_p\}$.
Therefore, we have $|V_\mathsf{oct} \cap Z_i| \leq hl/p$ for some $i \in [p]$.
Set $V' = V_\mathsf{oct} \cap Z_i$.
Since $V_\mathsf{oct} \subseteq S$, we have $V' \subseteq Z_i \cap S$.
Also, we have $V_\mathsf{oct} \cap (Z_i - V') = \emptyset$, which implies our claim.
With this claim, it now suffices to test, for every pair $(i,V')$ where $i \in [p]$ and $V' \subseteq Z_i \cap S$ is of size at most $hl/p$, whether $G[\gamma(t)]$ has a $(V_0,V_1,V_2)$-compatible OCT of size at most $l$ that is disjoint with $Z_i - V'$.

\begin{lemma}
Let $G$ be a graph, $Z \subseteq V(G)$, and $w = \mathbf{tw}(G/Z)$.
Given any $V_0,V_1,V_2 \subseteq V(G)$, one can compute in $w^{O(w)} \cdot |V(G)|^{O(1)}$ time a minimum-sized $(V_0,V_1,V_2)$-compatible OCT of $G$ that is contained in $V(G) - Z$ (or decide the non-existence of such an OCT).
\end{lemma}

\paragraph{Computing a progressive representative.}

\subsection{Proof of Lemma~\ref{lem-structure}} \label{sec-proofstr}

\section{OCT in unit-disk graphs}

\begin{lemma} \label{lem-structure1}
Given the representation of an $n$-vertex unit-disk graph $G$ and an integer $p \in [n]$, one can compute in $n^{O(1)}$ time a partition $\{V_1,\dots,V_p\}$ of $V(G)$ and a clique tree decomposition of $G/V_i$ with width $O(p)$ for each $i \in [p]$.
\end{lemma}

\subsection{Proof of Lemma~\ref{lem-structure1}}

Let $\langle \mathcal{D},k \rangle$ be the input of the problem, where $\mathcal{D}$ is a set of $n$ disks in the plane and $k$ is the parameter.
Let $G_\mathcal{D} = (\mathcal{D},E)$ be the unit-disk graph defined by $\mathcal{D}$.

\paragraph{The layering procedure.}
We compute a layering $\ell: \mathcal{D} \rightarrow \mathbb{N}$ of the disks as follows.
First, we build a grid $\varGamma$ consisting of squares with side-length $\frac{1}{2}$.
For a unit disk $D$, we use the notation $\Box_D$ to denote the cell of $\varGamma$ that contains the center of $D$.
Furthermore, for a cell $\Box$ of $\varGamma$ and a set $\mathcal{X}$ of unit disks, we use the notation $\mathcal{X}(\Box)$ to denote the subset of unit disks in $\mathcal{X}$ whose centers are in $\Box$.
Then our layering procedure is the following.

\begin{algorithm}[h]
    \caption{\textsc{Layering}$(\mathcal{D})$ \Comment{Output a layering $\ell: \mathcal{D} \rightarrow \mathbb{N}$}}
	\begin{algorithmic}[1]
        \State $t \leftarrow 0$
        \While{$\mathcal{D} \neq \emptyset$}
            \State $t \leftarrow t + 1$
            \State $\mathcal{D}_\mathsf{out} \leftarrow \{D \in \mathcal{D}: D \text{ is exposed on the outer boundary of } \bigcup_{D \in \mathcal{D}} D\}$
            \State $\mathcal{L} \leftarrow \bigcup_{D \in \mathcal{D}_\mathsf{out}} \mathcal{D}(\Box_D)$
            \State $\ell(D) \leftarrow \lceil t/100 \rceil$ for all $D \in \mathcal{L}$
            \State $\mathcal{D} \leftarrow \mathcal{D} \backslash \mathcal{L}$
        \EndWhile
        \State \textbf{return} $\ell$
	\end{algorithmic}
	\label{alg-layering}
\end{algorithm}

\paragraph{Basic properties of the layering.}
Let $\ell: \mathcal{D} \rightarrow \mathbb{N}$ be the layering of $\mathcal{D}$ obtained using the above algorithm.
For convenience, we write $\mathcal{L}_i = \ell^{-1}(\{i\})$ and call it \textit{the $i$-th layer}.
Suppose there are in total $m$ layers.
We define $\mathcal{L}_{>i} = \bigcup_{j=i+1}^m \mathcal{L}_j$ and $\mathcal{L}_{[i',i]} = \bigcup_{j=i'}^i \mathcal{L}_j$.
We now establish some basic properties of our layering.
\begin{lemma}
For any $D,D' \in \mathcal{D}$ such that $D \cap D' \neq \emptyset$, we have $|\ell(D) - \ell(D')| \leq 1$.
\end{lemma}

\begin{lemma}
Let $C$ be a connected component of $G[\mathcal{L}_{>i}]$.
Then $N(C) \cap \mathcal{L}_i$ lies in a connected component of $G[\mathcal{L}_i]$.
\end{lemma}

\begin{lemma}
The induced subgraph $G[\mathcal{L}_{[i',i]}]$ has tree width $O(s)$ after contracting the vertices in the same cell of $\varGamma$ into a single vertex, where $s = i'-i+1$.
\end{lemma}

\begin{fact}
Let $G = (V,E)$ be a connected unit-disk graph.
Then for any $V' \subseteq V$ of size $d$, the induced subgraph $G [V \backslash V']$ consists of $O(d)$ connected components.
\end{fact}

==> useless <==
\section{Introduction}
The study of subexponential time parameterized algorithms on planar and $H$-minor free graphs has been one of the most active sub-areas of parameterized algorithms, resulting in exciting results and powerful methods. Examples include Bidimensionality~\cite{demaine2005subexponential}, applications of Baker's layering technique~\cite{FominLMPPS1,DornFLRS13},\todo{what to cite} bounds on the treewidth of the solution~\cite{FominLKPS20,KleinM14,KleinM12,MarxPP18}, and pattern coverage~\cite{FominLMPPS16,Nederlof20a}. The central theme of all these results is that planar graphs exhibit the ``{\em square root phenomenon}'': parameterized problems whose fastest parameterized algorithm run in time $f(k)n^{O(k)}$ or $2^{O(k)}$ on general graphs admit $f(k)n^{O(\sqrt{k})}$ or even $2^{O(\sqrt{k})}n^{O(1)}$ time algorithms when input is restricted to planar or  $H$-minor free graphs.

Another central research direction within parameterized algorithms is the study of cut and cycle hitting problems such as {\sc Multiway Cut}, {\sc Multicut}, {\sc Odd Cycle Transversal} and {\sc Directed Feebdack Vertex Set}. The existence of $f(k)n^{O(1)}$ time algorithms for these problems were considered major open problems~\cite{DowneyF99}, and the algorithms developed for these problems~\cite{BousquetDT18,ChenLLOR08,MarxR14,Marx06,ReedSV04} and their generalizations~\cite{ChitnisCHPP16,ChitnisHM13,ChitnisCHM15,CyganKLPPSW21,CyganPPW13,GokeMM20,KratschPPW15,KimKPW21,LokshtanovMRS17,LokshtanovPSSZ20,MarxOR13,Wahlstrom17} have become standard textbook material~\cite{CyganFKLMPPS15}. 
%
Our paper is concerned with the following question: 
\begin{tcolorbox}
%{\em 
\begin{center}
Does the square root phenomenon apply to cut and cycle hitting problems?
\end{center}
%} 
\end{tcolorbox}
\smallskip
\noindent 
Despite substantial previous progress this question still remains largely unresolved. In fact, for most of these problems even an algorithm with running time $n^{O(\sqrt{k})}$  is not known, when input is restricted to planar or  $H$-minor free graphs. In this paper we make substantial progress on this question. 

%%\paragraph{Previous Work on Cut and Cycle Hitting Problems on Planar Graphs.}
\subsection{Previous Work on Cut and Cycle Hitting Problems on Planar Graphs}
%Problems arising from the domain of Cuts \& Connectivity hold a lot of promise and remain hitherto unexplored form the perspective of parameterized subexponential algorithms, with exceptions that are few and far between. 
In most cut problems, we have an input graph $G$, a set of terminals $T\subseteq V(G)$, a set 
 $R$ of unordered pairs of vertices in $T$, called terminal pairs, and a positive integer $k$, and the objective is to test whether we can delete at most $k$ edges (or vertices), say $S$, so that ``certain demands on  terminal pairs in $R$ are met''.  When we demand that  for every terminal pair 
 $(t_1,t_2)\in R$, the vertices $t_1$ and $t_2$ lie in different connected components of $G-S$, this corresponds to \probEMultiC. When the set $R$ of pairs of terminals comprises all the pairs of vertices in the set $T$ of terminals, it corresponds to \probEMC (also known as {\sc Multiterminal Cut}). Thus, naturally cut problems have three parameters: (a) size of the set of terminal ($r)$ (or the the number of request pairs); (b) the solution size $k$; and (c) the combined parameter $r+k$. 

Dahlhaus et al.~\cite{DahlhausJPSY94} initiated an algorithmic study of  \probEMC, and showed that the problem is NP-complete on general graphs  when $|T|\geq 3$, and  on planar graphs when $|T|$ is part of the input.  They complemented the result on planar graphs by designing an algorithm with running time $O((4r)^r n^{2r-1}\log n)$. Klein and Marx, revisited this problem in $2012$, and designed an algorithm with running time 
$2^{O(r)} n^{O(\sqrt{r})}$~\cite{KleinM12}. Marx~\cite{Marx12} also showed that, this algorithm is essentially tight. That, is they showed that the problem is W[1]-hard. In fact, Marx~\cite{Marx12} showed that unless Exponential Time Hypothesis (ETH), there is no algorithm solving the problem in time $f(r)n^{O(r)}$, for some function $f$ depending on $r$ alone.  de Verdi\`{e}re~\cite{Verdiere17} generlized this result to \probEMultiC and to graphs of genus $g$. In particular, 
%This result was extended by .. ~\cite{} to graphs of genus $g$ and to \probEMultiC. That is, .. ~\cite{} 
he designed an algorithm with running time $(g+r)^{O(g+r)} n^{O(\sqrt{g^2+gr})}$~\cite{Verdiere17}; which is shown to be optimal in~\cite{Cohen-AddadVMM19}. Finally, Cohen-Addad et al.~\cite{Cohen-AddadVM21} designed $(1+\epsilon)$ approximation algorithm 
for \probEMultiC running in time $(g+r)^{O((g+r)^3)} (\frac{1}{\epsilon})^{O(\sqrt{g+r})}n \log n$. In the last two results $r=|R|$. 

While, \probEMC and  \probEMultiC, parameterized by $|T$ and $|R|$, on planar graphs and graphs of bounded genus have been studied in literature, there is only one such result with respect to solution size $k$, as a parameter.  In a seminal result Pilipczuk et al.~\cite{PilipczukPSL18} designed a polynomial kernel for \probSteiner on graphs of bounded genus and utilized it together with a known algorithm to design $2^{O(\sqrt{k \log k})} n^{O(1)}$ time algorithm for \probSteiner on graphs of bounded genus. Using a duality between  \probSteiner  and \probEMC  on planar graphs, Pilipczuk et al.~\cite{PilipczukPSL18} also designed a polynomial kernel for \probEMC on planar graphs. Using this kernel they  designed  $2^{O(\sqrt{k} \log k)} n^{O(1)}$ time algorithm for \probEMC on planar graphs.

%This result can also be derived by an application of tools from Fomin et al.~\cite{}. 

A subexponential time algorithm for \probFVS (deleting vertices to hit all cycles) on $H$-minor free graphs  follows from the the theory of Bidimensionality~\cite{demaine2005subexponential}. However, if we are only interested in hitting odd cycles (\probOCT), theory of  Bidimensionality~\cite{demaine2005subexponential} does not apply.  Lokshtanov et al.~\cite{LokshtanovSW12} gave the first $2^{O(\sqrt{k} \log k)}n^{O(1)}$ time randomized algorithm for \probOCT on planar graphs. Later, Jansen et al.~\cite{JansenPL19} designed deterministic polynomial kernels for \probOCT and \probVMC. Using this kernel the algorithm of Lokshtanov et al.~\cite{LokshtanovSW12}  can be made deterministic. Finally, we would also like to mention results on {\sc Subset TSP}.  Marx et al.~\cite{MarxPP18}  $2^{O(\sqrt{k} \log k)} n^{O(1)}$ time algorithm for {\sc Subset TSP} on edge-weighted directed planar graphs. Earlier,  Klein and Marx~\cite{KleinM14} obtained a similar result for  {\sc Subset TSP}  on  undirected planar graphs.  


%\paragraph{Our results.}
\subsection{Our Results and Methods}
In this paper we make a significant step forward in understanding the parameterized complexity of cut and cycle hitting problems on $H$-minor free graphs. 

\smallskip
\begin{tcolorbox}
%{\em 
\begin{center}
We provide an algorithmic framework that allows us to design the first $n^{O(\sqrt{k})}$ time algorithm for several cut and cut and cycle hitting problems on $H$-minor free graphs in a uniform way. This includes  the first $n^{O(\sqrt{k})}$ time algorithm for \probEMC, \probVMC, \probEB, and \probOCT on 
$H$-minor free graphs. 

\end{center}
%} 
\end{tcolorbox}

\smallskip

Algorithms running in time $n^{O(\sqrt{k})}$ are subexponential but they are not parameterized  subexponential algorithms; that is they are not of the form $2^{o(k)}n^{O(1)}$.   We incorporate 
a notion of candidate sets, a notion weaker than polynomial kernels, in our framework and design parameterized  subexponential algorithms for several aforementioned problems.  A parameterized problem is said to admit a {\em  kernel}, if there is a polynomial time algorithm (the degree of polynomial is independent of $k$), called a kernelization algorithm, that reduces the input instance  $(I,k)$ down to an instance $(I',k')$ with size bounded by a function $p(k)$ in $k$, while preserving the answer. This reduced instance is called a $p(k)$ kernel for the problem. If $p(k)$ is (quasi)-polynomial  then we say 
that a paramterized problem admits a (quasi)-polynomial kernel~\cite{CyganFKLMPPS15,fomin2019kernelization}. Randomized kernels of 
(quasi)-polynomial size is known for several cut problems~\cite{KratschW14,KratschW20,HolsK18,Wahlstrom20,corr/abs-2002-08825} on general graphs. For these problems, 
it is natural to first apply the kernelization algorithm and then run the $n^{O(\sqrt{k})}$ time algorithm on the obtained kernel to design parameterized  subexponential algorithms. There are two difficulties with this approach. 
\begin{enumerate}
\setlength{\itemsep}{-2pt}
\item  Even though we start with a graph $G$ that excludes some fixed graph $H$ as a minor, it is not necessary that the output graph $G'$ will also exclude $H$ as a minor, as we are running a kernelization algorithm for general graphs. 
\item  The reduced parameter $k'$ could become $k^{O(1)}$, and thus running $n^{O(\sqrt{k})}$ time  algorithm on kernel may not yield the desired result. 
\end{enumerate}
 
In most of the know kernelization algorithm $k'\leq k$ and hence, the second difficulty can be overcome. However, the first constraint is more challenging and requires making the known kernelization algorithm return an instance in the desired family of graphs. That is, if $\cal G$ is the family of input graphs, then we would like the kernelization algorithm also to return the output graph $G' \in {\cal G}$. We overcome this difficulty by observing that known kernelization algorithm for cut problems can be made to output  a 
``candidate set'' of size (quasi)-polynomial in $k$. A candidate set is a set $\mathsf{Cand} \subseteq V(G)$ (resp., $\mathsf{Cand} \subseteq E(G)$), satisfying that 
$(I,k)$ has a solution of size at most $k$ if and only of $I$ has a solution of size at most $k$ that is contained in $\mathsf{Cand}$. By incorporating candidate set in our framework, we obtain the following parameterized  subexponential algorithms. 

%
%Let $I$ be an instance of a parameterized vertex-deletion (resp., edge-deletion) problem with graph $G$ and solution-size parameter $k \in \mathbb{N}$.
%A \textbf{candidate set} for $I$ is a set $\mathsf{Cand} \subseteq V(G)$ (resp., $\mathsf{Cand} \subseteq E(G)$) satisfying that $I$ has a solution of size at most $k$ iff $I$ has a solution of size at most $k$ that is contained in $\mathsf{Cand}$.

%parameterized  subexponential algorithms
%remedy this situation for se
%by utilizing a notion, weaker than
%This brings us to the notion of polynomial kernels.  
%Observe that if 
%any of the above mentioned problems admit a polynomial kernel (a polyn), or even a kernel of size $2^{o(k)}$. 


\begin{itemize}
\setlength{\itemsep}{-1pt}
\item In the \probOCT (resp., \probEB) problem input is a graph $G$ and integer $k$. The task is to determine whether there exists a set $S$ of at most $k$ vertices (resp., edges) so that $G - S$ is bipartite. 
We give a $2^{O(\sqrt{k}\log k)} \cdot n^{O(1)}$ time algorithm for \probOCT and for \probEB. 

\item In the \probVMC (resp., \probEMC) problem input is a graph $G$ a vertex set $T \subseteq V(G)$ of size $r$, and an integer $k$. The task is to determine whether there exists a set $S$ of at most $k$ vertices in $V(G) \setminus T$ (resp., edges in $E(G)$) such that no connected component of $G - S$ contains at least two vertices from $T$. We obtain a $2^{O(r \sqrt{k} \log k)} \cdot n^{O(1)}$ time algorithm for \probVMC and a $2^{O(\sqrt{k}\log^4 k)} \cdot n^{O(1)}$ time algorithm for \probEMC. Note that the running time of the algorithm for \probVMC depends on $r$ while the one for \probEMC does not. 

\item In the \probVMultiC (resp., \probEMultiC) problem input is a graph $G$, together with $r$ vertex pairs $(s_1, t_1), \ldots, (s_r, t_r)$. The task is to determine whether there exists a vertex subset $S \subseteq V(G) \setminus \{s_i, t_i ~:~ i \leq r\}$ (resp., edge subset $S \subseteq E(G)$) such that no connected component of $G - S$ contains both $s_i$ and $t_i$ for any $i \leq r$. We obtain a $2^{O((\sqrt{rk}+r) \log (rk))} \cdot n^{O(1)}$ time algorithm for \probVMultiC and a $2^{O((r+\sqrt{k})\log^4 (rk))} \cdot n^{O(1)}$ time algorithm for \probEMultiC.

\item In the \probGFVS (resp., \probGFES) problem input is a graph $G$, together with a function $\Lambda : V(G) \times V(G) \rightarrow \Sigma$ and an integer $k$, where $\Sigma$ is a group of size $g$ and $\Lambda$ satisfies $\Lambda(u,v) \times \Lambda(v,u) = \mathbf{1}$. The task is to determine whether there exists $S \subseteq V(G)$ (resp., $S \subseteq E(G)$) of size at most $k$ such that $G-S$ has no {\em non-null cycles}. Here a non-null cycle is a cycle $(v_0,v_1,\dots,v_m = v_0)$ in the graph satisfying $\prod_{i=1}^m \Lambda(v_{i-1},v_i) \neq \mathbf{1}$.
We obtain a $2^{O(g \sqrt{k}\log(gk))} \cdot n^{O(1)}$ time algorithm for \probGFVS and a $2^{O(\sqrt{k} \log g \log^4 k)} \cdot n^{O(1)}$ time algorithm for \probGFES.
\end{itemize}

For convenience, in the rest of the paper, we use the following abbreviations for the problem names: \probOCT (OCT), \probEB (EB), \probVMC (VMWC), \probEMC (EMWC), \probVMultiC (VMC), \probEMultiC (EMC), \probGFVS (GFVS), and \probGFES (GFES).


\paragraph{Methods.} 
\todo[inline]{Add some parallel with contraction theorem and ..}
All of our algorithms are based on what can be seen as a new version of the classical contraction decomposition theorem which has been used extensively to design parameterized and approximation algorithms.
For simplicity, let us only focus on planar graphs at this point.
The contraction decomposition theorem states that the edges of every planar graph can be partitioned into any prescribed number $p$ of
pieces such that contracting any piece results in a graph of $O(p)$ treewidth.
Our generalization can be expressed in the context of planar graphs as follows.

\begin{lemma}\label{lem:exposition}
Let $G$ be a planar graph.
Then for any $p \in \mathbb{N}$, there exist disjoint sets $Z_1,\dots,Z_p \subseteq V(G)$ such that for every $i \in [p]$ and every $Z' \subseteq Z_i$, $\mathbf{tw}(G/(Z_i \backslash Z')) = O(p+|Z'|)$.
Furthermore, the sets $Z_1, \dots, Z_p$ can be computed in polynomial times. 
\end{lemma}

Here $G/V$ denote the graph obtained from $G$ by contracting each edge in the induced subgraph $G[V]$.
%In other words, noting $E_i$ the set of edges in each $G[Z_i]$, then the $E_i$ for $i \in [p]$ are disjoint sets of edges such that $tw(G/ E_i) = O(p)$ for every $i \in [p]$.
%The only difference with the contraction decomposition theorem is that the $E_i$ are not a partition of the edges, however this property is usually not utilized in most applications of said theorem.
To see why the above lemma implies the contraction decomposition theorem, let $E_1,\dots,E_p$ be the edges in $G[Z_1],\dots,G[Z_p]$.
Since $Z_1, \dots, Z_p$ are disjoint, $E_1,\dots,E_p$ are also disjoint and thus there exists a partition $E_1',\dots,E_p'$ of the edges of $G$ such that $E_i \subseteq E_i'$.
Then we have $\mathbf{tw}(G/E_i') \leq \mathbf{tw}(G/E_i) = \mathbf{tw}(G/Z_i) = O(p)$.
A very important difference however is that, in our result, we still have control on the treewidth of the resulting graph, even if we do not contract all the edges of each $E_i$. 

To see an example where this difference is crucial, let us consider the \probEB problem on planar graphs, where the goal is to find a set $S$ of $k$ edges such that $G-S$ is bipartite. Using known techniques (see Lemma \ref{lem-candidate} below), we can find in polynomial time a set $\mathsf{Cand}$ of size $k^{O(1)}$ such that we only need to look inside $\mathsf{Cand}$ for the solution. Let $Z_1, \dots, Z_p$ be the sets obtain from applying Lemma \ref{lem:exposition} with $p = \sqrt{k}$, and $E_1,\dots,E_p$ be the sets of edges in $G[Z_1],\dots,G[Z_p]$. Because we are looking for a solution $S$ of size $k$ and $E_1,\dots,E_p$ are disjoint, it means that one of these sets, say $E_i$, contains less than $\sqrt{k}$ edges of $S$. As we are looking for a solution $S \subseteq \mathsf{Cand}$, there are at most $k^{O(\sqrt{k})}$ possible sets for $S_i :=S \cap E_i$. Therefore, by trying all the possibilities of $i$ and $S_i$, we can assume that the algorithm knows $S_i$. Denoting $Z'$ the set of vertices adjacent to edges in $S_i$, it means that we have $|Z'| = O(\sqrt{k})$ and thus our lemma implies that $\mathbf{tw}(G/(Z_i \setminus Z')) = O(\sqrt{k})$. A pretty standard DP argument shows that \probEB on a graph $H$ can be solved in time $2^{O(\mathbf{tw}(H))}n^{O(1)}$, and we will be able to adapt this argument to solve \probEB in $G$ in time $2^{O(\mathbf{tw}(G/(Z_i \setminus Z')))}n^{O(1)} = 2^{O(\sqrt{k})}n^{O(1)}$. Indeed, while some of the vertices in $G/(Z_i \setminus Z')$ can correspond to a large connected component $C$ of $G[Z_i \setminus Z']$, the fact that we have contracted only edges which are \textit{not} in the solution means that $C$ is bipartite, and in the DP we only have to guess which side of $C$ will belongs to which side of the final bipartition of $G-S$. 

A similar approach using only the contraction decomposition Theorem would fail, as it requires that one set completely avoids the solution. Therefore $p$ needs to be greater than $k$, and we obtain a decomposition of a graph after contraction of treewidth at least $k$, which cannot lead to a subexponential-time algorithm.

In order to prove Lemma \ref{lem:exposition} we will consider the vertex-face incidence (VFI) graph of $G$, which is a bipartite graph containing on one side the set of vertices of $G$ and on the other side the set of faces. Moreover, a vertex is adjacent to a face if it belongs to its boundary. Classically, if the VFI graph of a planar graph has diameter at most $p$, then $\mathbf{tw}(G) = O(p)$.
The \textit{deep} faces of $G$ refer to the faces farthest from the outer face $o$ of $G$, i.e., the faces have the maximum distance from $o$ in the VFI of $G$.
The following lemma is an essential part of our proof.

\begin{lemma}\label{lem:exposition_planar}
    Let $G$ be a planar graph such that the VFI graph of $G$ has diameter $p$.
    For each deep face $f$ of $G$, let $\kappa(f)$ be a set of at most $q$ vertices on the boundary of $f$.
%\begin{itemize}
%\item For every $i \in I$, $N(i)$ is included in the boundary  $\partial f_i$ of a face $f_i$ and $|N(i)| \leq t$;
%\item For every disjoint pair $i,j \in I$, the faces $f_i$ and $f_j$ are different.
%\end{itemize}
    Then there exists a tree decomposition of $G$ of width $O(p+q)$ where for every deep face $f$ of $G$, $\kappa(f)$ is contained in some bag of the decomposition. 
\end{lemma}

%Note that, since all the faces $f_i$ are different, we can easily see that the new graph $G'$ is planar, and that its VFI graph has diameter $O(p)$.
The key idea for proving the above lemma (without going into details) is the following.
We draw inside each deep face $f$ of $G$ a $|\kappa(f)| \times |\kappa(f)|$ grid and connecting the vertices in the first row of the grid to the vertices in $\kappa(f)$.
The resulting graph $G'$ is still planar.
Since the grids are drawn in the deep faces of $G$, the VFI graph of $G'$ has diameter $O(p+q)$, so there is a tree decomposition of $G'$ of width $O(p+q)$.
We then exploit the well-linked property of grids to show how to modify this tree decomposition (without significantly increasing its width) to force the vertices in each $\kappa(f)$ to be contained the same bag.
%The idea to obtain a decomposition of $O(p+q)$ will be to replace every $i \in I$ by some grid of order $O(|N(i)|)$ and use the well linked property of the grid to show that we can force the vertices of $\kappa(f)$ to belong to the same bag. 

With Lemma~\ref{lem:exposition_planar}, let us explain roughly how to obtain the sets $Z_1, \dots, Z_p$ of Lemma \ref{lem:exposition}. Let $G$ be a planar graph and assumed that the embedding is fixed. Consider now a BFS in the VFI graph of $G$ starting from the outer face. Let $L_0, L_1, \dots, L_m$ denote the different levels of the BFS. In particular, we will be interested in the odd levels $L_{2i + 1}= L'_i$ for $i \leq m/2$. As $L_0$ is the outer face and the VFI graph is bipartite, the $L'_i$ form a partition of the vertices of $G$. An interesting way to understand the $L'_i$ is by noting that $L'_1$ is exactly the boundary of the outer face of $G$, $L'_2$ is exactly the boundary of the outerface of $G - L'_1$ and so on.   

For every $i \in [p]$, we now define each $Z_i$ as the union of the $L'_j$ for $j = i \pmod p$. Let $Z'$ be a subset of vertices in $Z_i$. In order to understand what happens when we contract the edges of $G[Z_i \setminus Z']$, let us partition the graph into $G_{\leq} := G[L'_1 \cup \cdots \cup L'_i ]$ and $G_{>} := G[L'_{i+1} \cup \cdots \cup L'_{m/2} ]$ the rest. The idea is to apply some sort of inductive argument in $G_>$ and then combine the tree decomposition with the one of $G_{\leq}/(Z_i \setminus Z')$. First note that, because $G_{\leq}$ consists of the first $2i < 2p$ layers of the BFS in the VFI graph of $G$, we have that the diameter in the VFI graph of $G_{\leq}$ is a $O(p)$. Moreover, we know $L'_i$ is the outerface of $G[L'_{i} \cup \dots \cup L'_{m/2} ]$ which means that $L'_i$ is a cut between $G_{\leq}$ and $G_>$. Moreover, it means that every connected component of $G_>$ sits inside one face of $G_{\leq}$ whose boundary is a cycle of $L'_i$. Let $C_1, \dots, C_r$ denote the connected components of $G_>$ and $\partial_1, \dots, \partial_r$ the set of cycles bounding the associated faces $f_1,\dots,f_r$ (we assume here for simplification that $f_1,\dots,f_r$ are different, and it is easy to see that they are all deep faces of $G$).
As all the $\partial_i$ are inside $L_i$, it means that in $G/(Z_i \backslash Z')$, each $\partial_j$ will be contracted into a cycle $\partial'_j$ of size $1 + |Z' \cap \partial_j| = O(|Z'|)$.

The idea of the proof is then to compute inductively a tree decomposition for each $C_j/(Z_i \backslash Z')$ as well as $G_\leq/(Z_i \backslash Z')$ and merge then together. In order to do that efficiently, we require that each $\partial'_j$ appears in one bag of the decomposition of $G_\leq/(Z_i \backslash Z')$ so that we can append the tree decomposition of $C_j/(Z_i \backslash Z')$ to this bag. In order to obtain such a tree decomposition of $G_\leq/(Z_i \backslash Z')$ we will use Lemma \ref{lem:exposition_planar}.
We let $\kappa(f_j)$ include, for every vertex $v$ in the contracted cycle $\partial'_j$, a vertex in the cycle $\partial_j$ corresponding to $v$.
Thus, $|\kappa(f_j)| = |\partial'_j| = O(|Z'|)$.
By Lemma \ref{lem:exposition_planar}, $G_\leq$ has a tree decomposition of width $O(p+|Z'|)$ in which every $\kappa(f_j)$ is contained in some bag.
This tree decomposition then induces an $O(p+|Z'|)$-width tree decomposition of $G_\leq/(Z_i \backslash Z')$ in which every $\partial'_j$ is contained in some bag.
%Note that the neighborhood of each contracted $C_j$ is indeed $\partial'_j$ and since every $\partial'_j$ has size $O(|Z'|)$, we obtain a tree decomposition of width $O(p + |Z'|)$. 

So far we sketched our results in only the context of planar graphs.
Of course, our actual results are much more general, and require more technical proofs.
We prove Lemma~\ref{lem:exposition} for \textit{almost-embeddable} graphs, which is a class of graphs generalizing the class of bounded-genus graphs.
With this in hand, we solve our problems by doing dynamic programming on the famous ``almost-embeddable'' tree decomposition of an $H$-minor-free graph introduced by Robertson and Seymour \cite{robertson2003graph}.
Specifically, the generalized version of Lemma~\ref{lem:exposition} allows us to apply Baker's technique with a second-level dynamic programming to efficiently compute the DP table at each node of the Robertson-Seymour tree decomposition.

\paragraph{Organization.}
The rest of the paper is organized as follows.
In Section~\ref{sec:framework}, we present the generic framework for solving our problems on $H$-minor-free graphs, which all of our algorithms follow.
In Section~\ref{sec-keyproof}, we prove our main technical lemma (Lemma~\ref{lem-key}).
Finally, in Section~\ref{sec-app}, we apply our framework in Section~\ref{sec:framework} to solve each of our problems individually.
















\section{OCT in $H$-minor-free graphs}

Before describing our algorithm, we first introduce a generalization of the OCT problem, called \textit{constrained OCT}.

\begin{definition}
For a graph $G = (V,E)$ and a triple $(V_0,V_1,V_2)$ of subsets of $V$, we say an odd cycle transversal $V_\mathsf{oct}$ of $G$ is $(V_0,V_1,V_2)$-\textbf{compatible} if \textbf{(i)} $V_0 \subseteq V_\mathsf{oct}$ and \textbf{(ii)} $V_1 \backslash V_\mathsf{oct}$ and $V_2 \backslash V_\mathsf{oct}$ belong to different parts in the bipartite graph $G-V_\mathsf{oct}$.
\end{definition}
\begin{definition}[constrained OCT]
The \textbf{constrained OCT} problem is a parameterized problem in which each instance is a 5-tuple $(G,V_0,V_1,V_2,k)$ where $G$ is a graph, $V_0,V_1,V_2$ are three disjoint subsets of $V(G)$, and $k \in \mathbb{N}$ is the parameter, and the goal is to decide whether $G$ has an odd cycle transversal $V_\mathsf{oct}$ of size at most $k$ that $(V_0,V_1,V_2)$-compatible.
%\textbf{(i)} $V_0 \subseteq V_\mathsf{oct}$, $V_1 \subseteq I_1$, $V_2 \subseteq I_2$, \\
%\textbf{(ii)} $I_1$ and $I_2$ are independent sets in $G$, \\
%\textbf{(iii)} $|V_\mathsf{oct}| \leq k$.
\end{definition}

%Our main technical contribution is the following lemma, which plays an important role in our OCT algorithm for $H$-minor-free graphs.

%The proof of Lemma~\ref{lem-structure} will be given in Section~\ref{sec-proofstr}.
%Before this, let us first describe our OCT algorithm, assuming Lemma~\ref{lem-structure} holds.
Our OCT algorithm is obtained by (nontrivially) combining the ideas of Robertson-Seymour decomposition, recursive understanding, Baker's technique, and a technical lemma we establish about the structure of a graph that admits a good star decomposition (Lemma~\ref{lem-structure}).
Let $G$ be the input graph, which is $H$-minor-free.
Let $h > 0$ be the constant in Lemma~\ref{lem-rsdecomp} and $h'$ be the smallest integer that is larger than $|V(\mathsf{rep}(\mathcal{C}))|$ for any equivalence class $\mathcal{C}$ of $\equiv_\mathsf{oct}$ in $\mathcal{F}_{\subseteq [h]}$.

\paragraph{High-level framework.}
Algorithm~\ref{alg-OCT} presents the high-level framework of our algorithm.
The algorithm consists of an initialization step (Line~1), the main loop (Line~2-12), and a finalization step (Line~13).
In the initialization step, we compute an $(h,h')$-good tree decomposition $(T,\beta)$ for $G$ with adhesion size at most $h$ (together with the almost-embeddable structure of the torso of each internal node of $T$).
To this end, we first compute the Robertson-Seymour decomposition $(T_0,\beta)$ for $G$ (Lemma~\ref{lem-rsdecomp}), which has adhersion size at most $h$ and $h$-almost-embeddable torsos.
Then for each leaf $t \in T_0$, we add to $t$ a child $t'$ with bag $\beta(t') = \emptyset$; let $T$ be the resulting tree.
It is clear that $(T,\beta)$ is a tree decomposition of $G$ with adhesion size at most $h$.
Note that each leaf of $T$ has an empty bag and each internal node of $T$ is a node of $T_0$ (hence its torso is $h$-almost-embeddable).
So $(T,\beta)$ is $(h,0)$-good and thus an $(h,h')$-good.

The main loop (Line~2-12) is the heart of our algorithm.
Roughly speaking, during the loop, what we do is to iteratively \textit{simplify} the problem instance $(G,k)$.
That is, in each iteration, we generate a new instance $(G,k)$ from the old one such that the new instance is a YES-instance iff the old one is.
Meanwhile, we maintain the tree decomposition $(T,\beta)$ to guarantee that it is always an $(h,h')$-good tree decomposition of the current graph $G$ with adhesion size $h$.
A detailed discussion of the main loop will be given shortly.
Before this, we first discuss when the loop terminates and what we do in the finalization step.

We terminate the main loop when the problem instance $(G,k)$ becomes ``sufficiently simple'' in the sense that $|T| = 1$, i.e., the tree $T$ has only a root node (Line~2).
At this point, we reach the finalization step (Line~13), which simply solves the instance $(G,k)$ by \textit{brute-force}.
Why are we able to use brute-force when $|T| = 1$?
As mentioned before, $(T,\beta)$ is always an $(h,h')$-good tree decomposition of $G$.
When $|T|=1$, the bag $\beta(t)$ of the only node $t \in T$ is of size at most $h'$, because $t$ is a leaf and $(T,\beta)$ is $(h,h')$-good.
It follows that $G$ consists of a subgraph $G_0$ with $|V(G_0)| \leq h'$ and some isolated vertices.
Therefore, $(G,k)$ is a YES-instance iff $(G_0,k)$ is.
Since $|V(G_0)| \leq h'$, the instance $(G_0,k)$ can be solved in constant time by brute-force.

\begin{algorithm}[h]
    \caption{\textsc{OddCycleTransversal}$(G,k)$}
	\begin{algorithmic}[1]
        \State Compute an $(h,h')$-good tree decomposition $(T,\beta)$ of $G$ with adheresion size at most $h$
        %\State \textsc{Contract}$((T,\beta),h')$
        \While{$|T| \geq 2$}
            \State $t \leftarrow$ an internal node of $T$ whose children are all leaves
            %\State $X \leftarrow \gamma(t)$ and $B \leftarrow \sigma(t)$
            \State $\mathcal{I}_\mathsf{yes} \leftarrow \emptyset$
            \For{all $V_0,V_1,V_2 \subseteq \sigma(t)$ and all $l \in [k+h]$}
                \State Solve the constrained OCT instance $(G[\gamma(t)],V_0,V_1,V_2,l)$
                \If{$(G[\gamma(t)],V_0,V_1,V_2,l)$ is a YES-instance}
                    \State $\mathcal{I}_\mathsf{yes} \leftarrow \mathcal{I}_\mathsf{yes} \cup \{(G[\gamma(t)],V_0,V_1,V_2,l)\}$
                \EndIf
            \EndFor
            \If{$(G[\gamma(t)],\emptyset,\emptyset,\emptyset,k) \notin \mathcal{I}_\mathsf{yes}$}
                \textbf{return} NO
            \EndIf
            %\State $\lambda \leftarrow$ an arbitrary bijection from $\sigma(t)$ to $[|\sigma(t)|]$
            %\State view both $G[\gamma(t)]$ and $G[\gamma'(t)]$ as boundaried graphs in $\mathcal{F}_{[|\sigma(t)|]}$
            \State $(G^*,c) \leftarrow$ \textsc{Representative}$(G[\gamma(t)],\mathcal{I}_\mathsf{yes})$
            \State $G \leftarrow G^* \oplus G[\gamma'(t)]$ and $k \leftarrow k-c$
            \State Modify $(T,\beta)$ by replacing the subtree $T_t$ with a single node $t^*$ with $\beta(t^*) = V(G^*)$
            %\State \textsc{Contract}$((T,\beta),h')$
        \EndWhile
        \State Solve the instance $(G,k)$ by brute-force
        %\nolinenumbers
	\end{algorithmic}
	\label{alg-OCT}
\end{algorithm}

In what follows, we discuss the main loop in detail.
In each iteration of the loop, we first pick an (arbitrary) internal node $t \in T$ whose children are all leaves (Line~3).
Note that the subtree $T_t$ is a star.
Consider the induced subgraph $G[\gamma(t)]$.
Fix a bijection $\lambda: \sigma(t) \rightarrow [|\sigma(t)|]$.
We can view $G[\gamma(t)]$ as a boundaried graph in $\mathcal{F}_{[|\sigma(t)|]}$ with boundary $\sigma(t)$ and labeling $\lambda$.
%Similarly, the labeling $\lambda$ also makes $G[\gamma'(t)]$ a boundaried graph in $\mathcal{F}_{[|\sigma(t)|]}$, and we have $G = G[\gamma(t)] \oplus G[\gamma'(t)]$.
Our goal in this iteration is to compute a progressive representative of the equivalent class of $\equiv_\mathsf{oct}$ containing $G[\gamma(t)]$.
To this end, the critical step is to solve a set of constrained OCT instances on $G[\gamma(t)]$ (Line~5-8).
Specifically, we solve the instances $(G[\gamma(t)],V_0,V_1,V_2,l)$ for all $V_0,V_1,V_2 \subseteq \sigma(t)$ and all $l \in [k+h]$.
This is the most technical part of our algorithm, and the main idea is to exploit the fact that $G[\gamma(t)]$ has a $(h,h')$-good \textit{star} decomposition, which is $(T_t,\beta)$.
We shall establish a structural lemma (Lemma~\ref{lem-structure}) for graphs that admit a good star decomposition, which then allows us to apply Baker's technique and dynamic programming on tree decomposition to solve the problem.
After the constrained OCT instances are solved, we then include the YES-instances (Line~8) in $\mathcal{I}_\mathsf{yes}$.
If $(G[\gamma(t)],\emptyset,\emptyset,\emptyset,k) \notin \mathcal{I}_\mathsf{yes}$, then we can immediately conclude that $(G,k)$ is a NO-instance (Line~9), because $(G[\gamma(t)],k)$ is a NO-instance.
Otherwise, we use the information of $\mathcal{I}_\mathsf{yes}$ to compute a progressive representative of the equivalent class of $\equiv_\mathsf{oct}$ containing $G[\gamma(t)]$ and the corresponding transposition (Line~10).
Specifically, the sub-routine \textsc{Representative} takes $G[\gamma(t)]$ and $\mathcal{I}_\mathsf{yes}$ as input, and output a pair $(G^*,c)$ where $G^*$ is a progressive representative of the equivalent class containing $G[\gamma(t)]$ and $c \in \mathbb{Z}^+$ is the transposition from $G[\gamma(t)]$ to $G'$.
Note that $G = G[\gamma(t)] \oplus G[\gamma'(t)]$, if we regard $G[\gamma'(t)]$ as a boundaried graph with boundary $\sigma(t)$ and labeling $\lambda$.
Thus, by the definition of a progressive representative, we know that $(G,k)$ is a YES-instance of OCT iff $(G^* \oplus G[\gamma'(t)],k-c)$ is.
We then replace $(G,k)$ with $(G^* \oplus G[\gamma'(t)],k-c)$ (Line~11).
After this, we modify the tree decomposition $(T,\beta)$ by replacing the subtree $T_t$ with a single node $t^*$ with $\beta(t^*) = V(G^*)$ (Line~12).
It is easy to see that after the modification, $(T,\beta)$ is a tree decomposition of the new $G$, i.e., $G^* \oplus G[\gamma'(t)]$, which is still $(h,h')$-good and with adhesion size at most $h$.
Furthermore, $|T|$ strictly decreases after the modification.
Therefore, the loop will terminate in at most $m$ iterations, where $m$ is the initial size of $T$.
This directly implies the correctness of our algorithm.
Next, we discuss the only two missing pieces of our algorithm, which are \textbf{(1)} how to solve the instances on $G[\gamma(t)]$ (Line~6) and \textbf{(2)} how to compute the progressive representative $G^*$ and the transposition $c$ (Line~10).

\paragraph{Solving the instances on $G[\gamma(t)]$.}
Consider a constrained OCT instance $(G[\gamma(t)],V_0,V_1,V_2,l)$ where $V_0,V_1,V_2 \subseteq \sigma(t)$ and $l \in [k+h]$.
We want to test if there exists a $(V_0,V_1,V_2)$-compatible OCT of $G[\gamma(t)]$ of size at most $l$.
If $l < |V_0|$, then $(G[\gamma(t)],V_0,V_1,V_2,l)$ is clearly a NO-instance.
So assume $l \geq |V_0|$.
First, we notice that using Lemma~\ref{lem-candidate}, we are able to compute a small relevant set for the instance.
\begin{corollary} \label{cor-candidate}
We can compute in $|\gamma(t)|^{O(1)}$ time a set $S \subseteq \gamma(t)$ of size $l^{O(1)}$ such that with probability at least $1-1/2^{|\gamma(t)|}$, $G[\gamma(t)]$ has a $(V_0,V_1,V_2)$-compatible OCT of size $l$ iff $G$ has a $(V_0,V_1,V_2)$-compatible OCT of size $l$ that is contained in $S$.
\end{corollary}
\begin{proof}
Let $G'$ be the graph obtained from $G[\gamma(t)] - V_0$ by adding edges $(u,v)$ for all $u \in V_1 \backslash V_0$ and $v \in V_2 \backslash V_0$.
One can easily verify that a subset $U \subseteq V(G')$ is an OCT of $G'$ iff $U \cup V_0$ is a $(V_0,V_1,V_2)$-compatible OCT of $G[\gamma(t)]$.
Furthermore, every $(V_0,V_1,V_2)$-compatible OCT of $G[\gamma(t)]$ can be written as $U \cup V_0$ where $U$ is an OCT of $G'$.
In other words, the map $U \mapsto U \cup V_0$ gives a one-to-one correspondence between the OCTs of $G'$ and the $(V_0,V_1,V_2)$-compatible OCTs of $G[\gamma(t)]$.
Therefore, if we use the algorithm of Lemma~\ref{lem-candidate} to compute a set $S' \subseteq V(G')$ of size $(l-|V_0|)^{O(1)}$ such that $G'$ has an OCT of size $l-|V_0|$ iff $G'$ has an OCT of size $l-|V_0|$ that is contained in $S'$, then the set $S = S' \cup V_0$ satisfies the property that $G[\gamma(t)]$ has a $(V_0,V_1,V_2)$-compatible OCT of size $l$ iff $G$ has a $(V_0,V_1,V_2)$-compatible OCT of size $l$ that is contained in $S$.
\end{proof}

Let $S \subseteq \gamma(t)$ be the set in the above corollary.
As mentioned before, we shall exploit the fact that $G[\gamma(t)]$ has an $(h,h')$-good star decomposition with adhesion size $h$.
To this end, we establish the following technical lemma, whose proof is deferred to Section~\ref{sec-proofstr}.

\begin{lemma} \label{lem-structure}
Let $G$ be a graph admitting a $(c,c')$-good star decomposition with adhesion size $c''$ for some constants $c,c',c''$.
Then for any $p \in [n]$, there are $Z_1,\dots,Z_p \subseteq V(G)$ satisfying the following. \\
\textbf{(i)} Each vertex $v \in V(G)$ is contained in at most $c''$ sets in $\{Z_1,\dots,Z_p\}$. \\
\textbf{(ii)} For any $i \in [p]$ and $V' \subseteq Z_i$, $\mathbf{tw}(G/(Z_i-V')) = O(p+|V'|)$, where the constant hidden in the big-$O$ notation depends on $c,c',c''$. \\
%one can compute in $|V(G)|^{O(1)}$ time a tree decomposition of $G \backslash V'$ in which each bag contains $O(p)$ vertices in $V(G) \backslash V_i$ and intersects $O(p')$ connected component of $G[V_i \backslash V']$ where $p' = |V'|$. \\
Furthermore, if the good star decomposition of $G$ (and the almost-embeddable structure of the torso of the central bag) is given, then the above sets $Z_1,\dots,Z_p$ can be computed in $|V(G)|^{O(1)}$ time.
\end{lemma}

We apply the above lemma with $G = G[\gamma(t)]$ and $p = \lfloor\sqrt{l}\rfloor$, and obtain the sets $Z_1,\dots,Z_p \subseteq V(G[\gamma(t)]) = \gamma(t)$.
We claim that $G[\gamma(t)]$ has a $(V_0,V_1,V_2)$-compatible OCT of size at most $l$ iff for some $i \in [p]$ and $V' \subseteq Z_i \cap S$ with $|V'| \leq hl/p$, $G[\gamma(t)]$ has a $(V_0,V_1,V_2)$-compatible OCT of size at most $l$ that is \textit{disjoint} with $Z_i - V'$.
The ``if'' part is obvious.
To see the ``only if'' part, assume $G[\gamma(t)]$ has a $(V_0,V_1,V_2)$-compatible OCT of size at most $l$.
Then it has a $(V_0,V_1,V_2)$-compatible OCT $V_\mathsf{oct} \subseteq S$ of size at most $l$ by Corollary~\ref{cor-candidate}.
By the property \textbf{(i)} in Lemma~\ref{lem-structure}, each vertex $v \in \gamma(t)$ is contained in at most $h$ sets in $\{Z_1,\dots,Z_p\}$.
Therefore, we have $|V_\mathsf{oct} \cap Z_i| \leq hl/p$ for some $i \in [p]$.
Set $V' = V_\mathsf{oct} \cap Z_i$.
Since $V_\mathsf{oct} \subseteq S$, we have $V' \subseteq Z_i \cap S$.
Also, we have $V_\mathsf{oct} \cap (Z_i - V') = \emptyset$, which implies our claim.
With this claim, it now suffices to test, for every pair $(i,V')$ where $i \in [p]$ and $V' \subseteq Z_i \cap S$ is of size at most $hl/p$, whether $G[\gamma(t)]$ has a $(V_0,V_1,V_2)$-compatible OCT of size at most $l$ that is disjoint with $Z_i - V'$.

\begin{lemma}
Let $G$ be a graph, $Z \subseteq V(G)$, and $w = \mathbf{tw}(G/Z)$.
Given any $V_0,V_1,V_2 \subseteq V(G)$, one can compute in $w^{O(w)} \cdot |V(G)|^{O(1)}$ time a minimum-sized $(V_0,V_1,V_2)$-compatible OCT of $G$ that is contained in $V(G) - Z$ (or decide the non-existence of such an OCT).
\end{lemma}

\paragraph{Computing a progressive representative.}

\subsection{Proof of Lemma~\ref{lem-structure}} \label{sec-proofstr}

\section{OCT in unit-disk graphs}

\begin{lemma} \label{lem-structure1}
Given the representation of an $n$-vertex unit-disk graph $G$ and an integer $p \in [n]$, one can compute in $n^{O(1)}$ time a partition $\{V_1,\dots,V_p\}$ of $V(G)$ and a clique tree decomposition of $G/V_i$ with width $O(p)$ for each $i \in [p]$.
\end{lemma}

\subsection{Proof of Lemma~\ref{lem-structure1}}

Let $\langle \mathcal{D},k \rangle$ be the input of the problem, where $\mathcal{D}$ is a set of $n$ disks in the plane and $k$ is the parameter.
Let $G_\mathcal{D} = (\mathcal{D},E)$ be the unit-disk graph defined by $\mathcal{D}$.

\paragraph{The layering procedure.}
We compute a layering $\ell: \mathcal{D} \rightarrow \mathbb{N}$ of the disks as follows.
First, we build a grid $\varGamma$ consisting of squares with side-length $\frac{1}{2}$.
For a unit disk $D$, we use the notation $\Box_D$ to denote the cell of $\varGamma$ that contains the center of $D$.
Furthermore, for a cell $\Box$ of $\varGamma$ and a set $\mathcal{X}$ of unit disks, we use the notation $\mathcal{X}(\Box)$ to denote the subset of unit disks in $\mathcal{X}$ whose centers are in $\Box$.
Then our layering procedure is the following.

\begin{algorithm}[h]
    \caption{\textsc{Layering}$(\mathcal{D})$ \Comment{Output a layering $\ell: \mathcal{D} \rightarrow \mathbb{N}$}}
	\begin{algorithmic}[1]
        \State $t \leftarrow 0$
        \While{$\mathcal{D} \neq \emptyset$}
            \State $t \leftarrow t + 1$
            \State $\mathcal{D}_\mathsf{out} \leftarrow \{D \in \mathcal{D}: D \text{ is exposed on the outer boundary of } \bigcup_{D \in \mathcal{D}} D\}$
            \State $\mathcal{L} \leftarrow \bigcup_{D \in \mathcal{D}_\mathsf{out}} \mathcal{D}(\Box_D)$
            \State $\ell(D) \leftarrow \lceil t/100 \rceil$ for all $D \in \mathcal{L}$
            \State $\mathcal{D} \leftarrow \mathcal{D} \backslash \mathcal{L}$
        \EndWhile
        \State \textbf{return} $\ell$
	\end{algorithmic}
	\label{alg-layering}
\end{algorithm}

\paragraph{Basic properties of the layering.}
Let $\ell: \mathcal{D} \rightarrow \mathbb{N}$ be the layering of $\mathcal{D}$ obtained using the above algorithm.
For convenience, we write $\mathcal{L}_i = \ell^{-1}(\{i\})$ and call it \textit{the $i$-th layer}.
Suppose there are in total $m$ layers.
We define $\mathcal{L}_{>i} = \bigcup_{j=i+1}^m \mathcal{L}_j$ and $\mathcal{L}_{[i',i]} = \bigcup_{j=i'}^i \mathcal{L}_j$.
We now establish some basic properties of our layering.
\begin{lemma}
For any $D,D' \in \mathcal{D}$ such that $D \cap D' \neq \emptyset$, we have $|\ell(D) - \ell(D')| \leq 1$.
\end{lemma}

\begin{lemma}
Let $C$ be a connected component of $G[\mathcal{L}_{>i}]$.
Then $N(C) \cap \mathcal{L}_i$ lies in a connected component of $G[\mathcal{L}_i]$.
\end{lemma}

\begin{lemma}
The induced subgraph $G[\mathcal{L}_{[i',i]}]$ has tree width $O(s)$ after contracting the vertices in the same cell of $\varGamma$ into a single vertex, where $s = i'-i+1$.
\end{lemma}

\begin{fact}
Let $G = (V,E)$ be a connected unit-disk graph.
Then for any $V' \subseteq V$ of size $d$, the induced subgraph $G [V \backslash V']$ consists of $O(d)$ connected components.
\end{fact}
